Symmetry reduction of gravitational Lagrangians

We analyze all possible symmetry reductions of Lagrangians that yield fully equivalent field equations for any 4-dimensional metric theory of gravity. Specifically, we present a complete list of infinitesimal group actions obeying the principle of symmetric criticality, identify the corresponding invariant metrics (and $l$-chains), discuss relations among them, and analyze simplifications allowed by the residual diffeomorphism group and Noether identities before and after variation of the reduced Lagrangian. We employ rigorous treatment of the symmetry reduction by Fels and Torre and use the Hicks classification of infinitesimal group actions by means of Lie algebras pairs of isometries and their isotropy subalgebras. The classification is recast in the coordinates in which the well-known symmetries and geometries are easily recognizable and relatable to each other. The paper is accompanied by a code for the symmetry reduction of Lagrangians that we developed in \texttt{xAct} package of \textsc{Mathematica}.

==> exported_arrays <==
KVarray = <|{3, 2, 1} -> {CTensor[{0, 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{0, 0, -y4[], y3[]}, {yCoords}, 0][a]}, 
    {3, 2, 2} -> {CTensor[{0, 0, Cos[y4[]], -(Coth[y3[]]*Sin[y4[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, -Sin[y4[]], 
         -(Cos[y4[]]*Coth[y3[]])}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a]}, 
    {3, 2, 3} -> {CTensor[{0, 0, Cos[y4[]], -(Cot[y3[]]*Sin[y4[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, -Sin[y4[]], -(Cos[y4[]]*Cot[y3[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, 0, 1}, {yCoords}, 0][a]}, 
    {3, 2, 4} -> {CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 1, 0, 0}, {yCoords}, 0][a], 
      CTensor[{y2[], y1[], 0, 0}, {yCoords}, 0][a]}, 
    {3, 2, 5} -> {CTensor[{-(Sin[y1[]]*Tanh[y2[]]), Cos[y1[]], 0, 0}, 
        {yCoords}, 0][a], CTensor[{-(Cos[y1[]]*Tanh[y2[]]), -Sin[y1[]], 0, 
         0}, {yCoords}, 0][a], CTensor[{1, 0, 0, 0}, {yCoords}, 0][a]}, 
    {3, 3, 2} -> {CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 1, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a]}, 
    {3, 3, 3} -> {CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{y4[], 0, 1, 0}, {yCoords}, 0][a]}, 
    {3, 3, 8} -> {CTensor[{-(Csch[y3[]]*Sin[y4[]]), 0, Cos[y4[]], 
         -(Coth[y3[]]*Sin[y4[]])}, {yCoords}, 0][a], 
      CTensor[{-(Cos[y4[]]*Csch[y3[]]), 0, -Sin[y4[]], 
         -(Cos[y4[]]*Coth[y3[]])}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a]}, 
    {3, 3, 9} -> {CTensor[{-(Csc[y3[]]*Sin[y4[]]), 0, Cos[y4[]], 
         -(Cot[y3[]]*Sin[y4[]])}, {yCoords}, 0][a], 
      CTensor[{-(Cos[y4[]]*Csc[y3[]]), 0, -Sin[y4[]], 
         -(Cos[y4[]]*Cot[y3[]])}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a]}, 
    {4, 3, 1} -> {CTensor[{0, 0, Cos[y4[]], -(Coth[y3[]]*Sin[y4[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, -Sin[y4[]], 
         -(Cos[y4[]]*Coth[y3[]])}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{1, 0, 0, 0}, {yCoords}, 0][a]}, 
    {4, 3, 2} -> {CTensor[{-(Csch[y3[]]*Sin[y4[]]), 0, Cos[y4[]], 
         -(Coth[y3[]]*Sin[y4[]])}, {yCoords}, 0][a], 
      CTensor[{-(Cos[y4[]]*Csch[y3[]]), 0, -Sin[y4[]], 
         -(Cos[y4[]]*Coth[y3[]])}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{1, 0, 0, 0}, {yCoords}, 0][a]}, 
    {4, 3, 3} -> {CTensor[{0, 0, Cos[y4[]], -(Cot[y3[]]*Sin[y4[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, -Sin[y4[]], -(Cos[y4[]]*Cot[y3[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{1, 0, 0, 0}, {yCoords}, 0][a]}, 
    {4, 3, 4} -> {CTensor[{-(Csc[y3[]]*Sin[y4[]]), 0, Cos[y4[]], 
         -(Cot[y3[]]*Sin[y4[]])}, {yCoords}, 0][a], 
      CTensor[{-(Cos[y4[]]*Csc[y3[]]), 0, -Sin[y4[]], 
         -(Cos[y4[]]*Cot[y3[]])}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{1, 0, 0, 0}, {yCoords}, 0][a]}, 
    {4, 3, 5} -> {CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{y4[], 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{(-y3[]^2 + y4[]^2)/2, 0, y4[], -y3[]}, {yCoords}, 0][a]}, 
    {4, 3, 6} -> {CTensor[{0, 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{0, 0, -y4[], y3[]}, {yCoords}, 0][a], 
      CTensor[{1, 0, 0, 0}, {yCoords}, 0][a]}, 
    {4, 3, 8} -> {CTensor[{-(Sin[y1[]]*Tanh[y2[]]), Cos[y1[]], 0, 0}, 
        {yCoords}, 0][a], CTensor[{-(Cos[y1[]]*Tanh[y2[]]), -Sin[y1[]], 0, 
         0}, {yCoords}, 0][a], CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a]}, 
    {4, 3, 9} -> {CTensor[{-(Sin[y1[]]*Tanh[y2[]]), Cos[y1[]], 
         -(Sech[y2[]]*Sin[y1[]]), 0}, {yCoords}, 0][a], 
      CTensor[{-(Cos[y1[]]*Tanh[y2[]]), -Sin[y1[]], -(Cos[y1[]]*Sech[y2[]]), 
         0}, {yCoords}, 0][a], CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 1, 0}, {yCoords}, 0][a]}, 
    {4, 3, 10} -> {CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{y4[], 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, y3[], -y4[]}, {yCoords}, 0][a]}, 
    {4, 3, 11} -> {CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 1, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{y2[], y1[], 0, 0}, {yCoords}, 0][a]}, 
    {4, 4, 1} -> {CTensor[{-(Csc[y3[]]*Sin[y4[]]), 0, Cos[y4[]], 
         -(Cot[y3[]]*Sin[y4[]])}, {yCoords}, 0][a], 
      CTensor[{-(Cos[y4[]]*Csc[y3[]]), 0, -Sin[y4[]], 
         -(Cos[y4[]]*Cot[y3[]])}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{0, 1, 0, 0}, {yCoords}, 0][a]}, 
    {4, 4, 2} -> {CTensor[{-(Csch[y3[]]*Sin[y4[]]), 0, Cos[y4[]], 
         -(Coth[y3[]]*Sin[y4[]])}, {yCoords}, 0][a], 
      CTensor[{-(Cos[y4[]]*Csch[y3[]]), 0, -Sin[y4[]], 
         -(Cos[y4[]]*Coth[y3[]])}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{0, 1, 0, 0}, {yCoords}, 0][a]}, 
    {4, 4, 9} -> {CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 1, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{-y4[], 0, 1, y2[]}, {yCoords}, 0][a]}, 
    {4, 4, 18} -> {CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{y4[], 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{0, 1, -y3[], y4[]}, {yCoords}, 0][a]}, 
    {4, 4, 22} -> {CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{y4[], 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{(-y3[]^2 + y4[]^2)/2, 1, y4[], -y3[]}, {yCoords}, 0][a]}, 
    {5, 4, 1} -> {CTensor[{-(Csch[y3[]]*Sin[y4[]]), 0, Cos[y4[]], 
         -(Coth[y3[]]*Sin[y4[]])}, {yCoords}, 0][a], 
      CTensor[{-(Cos[y4[]]*Csch[y3[]]), 0, -Sin[y4[]], 
         -(Cos[y4[]]*Coth[y3[]])}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 1, 0, 0}, {yCoords}, 0][a]}, 
    {5, 4, 2} -> {CTensor[{-(Csc[y3[]]*Sin[y4[]]), 0, Cos[y4[]], 
         -(Cot[y3[]]*Sin[y4[]])}, {yCoords}, 0][a], 
      CTensor[{-(Cos[y4[]]*Csc[y3[]]), 0, -Sin[y4[]], 
         -(Cos[y4[]]*Cot[y3[]])}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 1, 0, 0}, {yCoords}, 0][a]}, 
    {5, 4, 3} -> {CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{y4[], 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{(-y3[]^2 + y4[]^2)/2, 0, y4[], -y3[]}, {yCoords}, 0][a], 
      CTensor[{0, 1, 0, 0}, {yCoords}, 0][a]}, 
    {5, 4, 6} -> {CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{y4[], 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, y3[], -y4[]}, {yCoords}, 0][a], 
      CTensor[{0, 1, 0, 0}, {yCoords}, 0][a]}, 
    {5, 4, 7} -> {CTensor[{-(Sin[y1[]]*Tanh[y2[]]), Cos[y1[]], 
         -(Sech[y2[]]*Sin[y1[]]), 0}, {yCoords}, 0][a], 
      CTensor[{-(Cos[y1[]]*Tanh[y2[]]), -Sin[y1[]], -(Cos[y1[]]*Sech[y2[]]), 
         0}, {yCoords}, 0][a], CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a]}, 
    {6, 3, 1} -> {CTensor[{0, 0, Cos[y4[]], -(Cot[y3[]]*Sin[y4[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, -Sin[y4[]], -(Cos[y4[]]*Cot[y3[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{0, Cos[y4[]]*Sin[y3[]], Cos[y3[]]*Cos[y4[]]*Cot[y2[]], 
         -(Cot[y2[]]*Csc[y3[]]*Sin[y4[]])}, {yCoords}, 0][a], 
      CTensor[{0, Sin[y3[]]*Sin[y4[]], Cos[y3[]]*Cot[y2[]]*Sin[y4[]], 
         Cos[y4[]]*Cot[y2[]]*Csc[y3[]]}, {yCoords}, 0][a], 
      CTensor[{0, Cos[y3[]], -(Cot[y2[]]*Sin[y3[]]), 0}, {yCoords}, 0][a]}, 
    {6, 3, 2} -> {CTensor[{0, 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{0, 0, -y4[], y3[]}, {yCoords}, 0][a], 
      CTensor[{0, y4[], 0, -y2[]}, {yCoords}, 0][a], 
      CTensor[{0, y3[], -y2[], 0}, {yCoords}, 0][a], 
      CTensor[{0, -1, 0, 0}, {yCoords}, 0][a]}, 
    {6, 3, 3} -> {CTensor[{0, 0, Cos[y4[]], -(Cot[y3[]]*Sin[y4[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, -Sin[y4[]], -(Cos[y4[]]*Cot[y3[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{0, Cos[y4[]]*Sin[y3[]], Cos[y3[]]*Cos[y4[]]*Coth[y2[]], 
         -(Coth[y2[]]*Csc[y3[]]*Sin[y4[]])}, {yCoords}, 0][a], 
      CTensor[{0, Sin[y3[]]*Sin[y4[]], Cos[y3[]]*Coth[y2[]]*Sin[y4[]], 
         Cos[y4[]]*Coth[y2[]]*Csc[y3[]]}, {yCoords}, 0][a], 
      CTensor[{0, Cos[y3[]], -(Coth[y2[]]*Sin[y3[]]), 0}, {yCoords}, 0][a]}, 
    {6, 3, 4} -> {CTensor[{-(Sin[y1[] - y3[]]*Tanh[y2[]]), Cos[y1[] - y3[]], 
         Coth[y2[]]*Sin[y1[] - y3[]], 0}, {yCoords}, 0][a], 
      CTensor[{Cos[y1[] - y3[]]*Tanh[y2[]], Sin[y1[] - y3[]], 
         -(Cos[y1[] - y3[]]*Coth[y2[]]), 0}, {yCoords}, 0][a], 
      CTensor[{-1, 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{Sin[y1[] + y3[]]*Tanh[y2[]], -Cos[y1[] + y3[]], 
         Coth[y2[]]*Sin[y1[] + y3[]], 0}, {yCoords}, 0][a], 
      CTensor[{Cos[y1[] + y3[]]*Tanh[y2[]], Sin[y1[] + y3[]], 
         Cos[y1[] + y3[]]*Coth[y2[]], 0}, {yCoords}, 0][a], 
      CTensor[{1, 0, 1, 0}, {yCoords}, 0][a]}, 
    {6, 3, 5} -> {CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 1, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{y2[], y1[], 0, 0}, {yCoords}, 0][a], 
      CTensor[{y4[], 0, 0, y1[]}, {yCoords}, 0][a], 
      CTensor[{0, -y4[], 0, y2[]}, {yCoords}, 0][a]}, 
    {6, 3, 6} -> {CTensor[{0, Cos[y3[]], -(Cot[y2[]]*Sin[y3[]]), 0}, 
        {yCoords}, 0][a], CTensor[{0, -Sin[y3[]], -(Cos[y3[]]*Cot[y2[]]), 0}, 
        {yCoords}, 0][a], CTensor[{0, 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{Cos[y3[]]*Sin[y2[]], Cos[y2[]]*Cos[y3[]]*Tanh[y1[]], 
         -(Csc[y2[]]*Sin[y3[]]*Tanh[y1[]]), 0}, {yCoords}, 0][a], 
      CTensor[{Sin[y2[]]*Sin[y3[]], Cos[y2[]]*Sin[y3[]]*Tanh[y1[]], 
         Cos[y3[]]*Csc[y2[]]*Tanh[y1[]], 0}, {yCoords}, 0][a], 
      CTensor[{Cos[y2[]], -(Sin[y2[]]*Tanh[y1[]]), 0, 0}, {yCoords}, 0][a]}, 
    {6, 4, 1} -> {CTensor[{0, 0, Cos[y4[]], -(Cot[y3[]]*Sin[y4[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, -Sin[y4[]], -(Cos[y4[]]*Cot[y3[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{-(Sin[y1[]]*Tanh[y2[]]), Cos[y1[]], 0, 0}, {yCoords}, 0][a], 
      CTensor[{-(Cos[y1[]]*Tanh[y2[]]), -Sin[y1[]], 0, 0}, {yCoords}, 0][a], 
      CTensor[{1, 0, 0, 0}, {yCoords}, 0][a]}, 
    {6, 4, 2} -> {CTensor[{0, 0, Cos[y4[]], -(Coth[y3[]]*Sin[y4[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, -Sin[y4[]], 
         -(Cos[y4[]]*Coth[y3[]])}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{-(Sin[y1[]]*Tanh[y2[]]), Cos[y1[]], 0, 0}, {yCoords}, 0][a], 
      CTensor[{-(Cos[y1[]]*Tanh[y2[]]), -Sin[y1[]], 0, 0}, {yCoords}, 0][a], 
      CTensor[{1, 0, 0, 0}, {yCoords}, 0][a]}, 
    {6, 4, 3} -> {CTensor[{-(Sin[y1[]]*Tanh[y2[]]), Cos[y1[]], 0, 0}, 
        {yCoords}, 0][a], CTensor[{-(Cos[y1[]]*Tanh[y2[]]), -Sin[y1[]], 0, 
         0}, {yCoords}, 0][a], CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{0, 0, -y4[], y3[]}, {yCoords}, 0][a]}, 
    {6, 4, 4} -> {CTensor[{0, 0, Cos[y4[]], -(Cot[y3[]]*Sin[y4[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, -Sin[y4[]], -(Cos[y4[]]*Cot[y3[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 1, 0, 0}, {yCoords}, 0][a], 
      CTensor[{y2[], y1[], 0, 0}, {yCoords}, 0][a]}, 
    {6, 4, 5} -> {CTensor[{0, 0, Cos[y4[]], -(Coth[y3[]]*Sin[y4[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, -Sin[y4[]], 
         -(Cos[y4[]]*Coth[y3[]])}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{y2[], y1[], 0, 0}, {yCoords}, 0][a], 
      CTensor[{1, 0, 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 1, 0, 0}, {yCoords}, 0][a]}, 
    {7, 4, 1} -> {CTensor[{0, 0, Cos[y4[]], -(Cot[y3[]]*Sin[y4[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, -Sin[y4[]], -(Cos[y4[]]*Cot[y3[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{0, Cos[y4[]]*Sin[y3[]], Cos[y3[]]*Cos[y4[]]*Cot[y2[]], 
         -(Cot[y2[]]*Csc[y3[]]*Sin[y4[]])}, {yCoords}, 0][a], 
      CTensor[{0, Sin[y3[]]*Sin[y4[]], Cos[y3[]]*Cot[y2[]]*Sin[y4[]], 
         Cos[y4[]]*Cot[y2[]]*Csc[y3[]]}, {yCoords}, 0][a], 
      CTensor[{0, Cos[y3[]], -(Cot[y2[]]*Sin[y3[]]), 0}, {yCoords}, 0][a], 
      CTensor[{1, 0, 0, 0}, {yCoords}, 0][a]}, 
    {7, 4, 2} -> {CTensor[{0, 0, Cos[y4[]], -(Cot[y3[]]*Sin[y4[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, -Sin[y4[]], -(Cos[y4[]]*Cot[y3[]])}, 
        {yCoords}, 0][a], CTensor[{0, 0, 0, 1}, {yCoords}, 0][a], 
      CTensor[{0, Cos[y4[]]*Sin[y3[]], Cos[y3[]]*Cos[y4[]]*Coth[y2[]], 
         -(Coth[y2[]]*Csc[y3[]]*Sin[y4[]])}, {yCoords}, 0][a], 
      CTensor[{0, Sin[y3[]]*Sin[y4[]], Cos[y3[]]*Coth[y2[]]*Sin[y4[]], 
         Cos[y4[]]*Coth[y2[]]*Csc[y3[]]}, {yCoords}, 0][a], 
      CTensor[{0, Cos[y3[]], -(Coth[y2[]]*Sin[y3[]]), 0}, {yCoords}, 0][a], 
      CTensor[{1, 0, 0, 0}, {yCoords}, 0][a]}, 
    {7, 4, 3} -> {CTensor[{0, Cos[y3[]], -(Cot[y2[]]*Sin[y3[]]), 0}, 
        {yCoords}, 0][a], CTensor[{0, -Sin[y3[]], -(Cos[y3[]]*Cot[y2[]]), 0}, 
        {yCoords}, 0][a], CTensor[{0, 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{Cos[y3[]]*Sin[y2[]], Cos[y2[]]*Cos[y3[]]*Tanh[y1[]], 
         -(Csc[y2[]]*Sin[y3[]]*Tanh[y1[]]), 0}, {yCoords}, 0][a], 
      CTensor[{Sin[y2[]]*Sin[y3[]], Cos[y2[]]*Sin[y3[]]*Tanh[y1[]], 
         Cos[y3[]]*Csc[y2[]]*Tanh[y1[]], 0}, {yCoords}, 0][a], 
      CTensor[{Cos[y2[]], -(Sin[y2[]]*Tanh[y1[]]), 0, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a]}, 
    {7, 4, 4} -> {CTensor[{-(Sin[y1[] - y3[]]*Tanh[y2[]]), Cos[y1[] - y3[]], 
         Coth[y2[]]*Sin[y1[] - y3[]], 0}, {yCoords}, 0][a], 
      CTensor[{Cos[y1[] - y3[]]*Tanh[y2[]], Sin[y1[] - y3[]], 
         -(Cos[y1[] - y3[]]*Coth[y2[]]), 0}, {yCoords}, 0][a], 
      CTensor[{-1, 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{Sin[y1[] + y3[]]*Tanh[y2[]], -Cos[y1[] + y3[]], 
         Coth[y2[]]*Sin[y1[] + y3[]], 0}, {yCoords}, 0][a], 
      CTensor[{Cos[y1[] + y3[]]*Tanh[y2[]], Sin[y1[] + y3[]], 
         Cos[y1[] + y3[]]*Coth[y2[]], 0}, {yCoords}, 0][a], 
      CTensor[{1, 0, 1, 0}, {yCoords}, 0][a], 
      CTensor[{0, 0, 0, 1}, {yCoords}, 0][a]}|>
ginvvarray = <|{3, 2, 1} -> CTensor[{f1[y1[], y2[]], f2[y1[], y2[]], 0, 0}, 
       {yCoords}, 0][a], {3, 2, 2} -> 
     CTensor[{f1[y1[], y2[]], f2[y1[], y2[]], 0, 0}, {yCoords}, 0][a], 
    {3, 2, 3} -> CTensor[{f1[y1[], y2[]], f2[y1[], y2[]], 0, 0}, {yCoords}, 
       0][a], {3, 2, 4} -> CTensor[{0, 0, f1[y3[], y4[]], f2[y3[], y4[]]}, 
       {yCoords}, 0][a], {3, 2, 5} -> 
     CTensor[{0, 0, f1[y3[], y4[]], f2[y3[], y4[]]}, {yCoords}, 0][a], 
    {3, 3, 2} -> CTensor[{f1[y3[]], f2[y3[]], f3[y3[]], f4[y3[]]}, {yCoords}, 
       0][a], {3, 3, 3} -> CTensor[{f1[y2[]] + f4[y2[]]*y3[], f2[y2[]], 
        f3[y2[]], f4[y2[]]}, {yCoords}, 0][a], 
    {3, 3, 8} -> CTensor[{f1[y2[]] + Coth[y3[]]*(Cos[y1[]]*f3[y2[]] - 
           f4[y2[]]*Sin[y1[]]), f2[y2[]], Cos[y1[]]*f4[y2[]] + 
         f3[y2[]]*Sin[y1[]], Csch[y3[]]*(Cos[y1[]]*f3[y2[]] - 
          f4[y2[]]*Sin[y1[]])}, {yCoords}, 0][a], 
    {3, 3, 9} -> CTensor[{f1[y2[]] + Cot[y3[]]*(Cos[y1[]]*f3[y2[]] - 
           f4[y2[]]*Sin[y1[]]), f2[y2[]], Cos[y1[]]*f4[y2[]] + 
         f3[y2[]]*Sin[y1[]], Csc[y3[]]*(Cos[y1[]]*f3[y2[]] - 
          f4[y2[]]*Sin[y1[]])}, {yCoords}, 0][a], 
    {4, 3, 1} -> CTensor[{f1[y2[]], f2[y2[]], 0, 0}, {yCoords}, 0][a], 
    {4, 3, 2} -> CTensor[{f1[y2[]], f2[y2[]], 0, 0}, {yCoords}, 0][a], 
    {4, 3, 3} -> CTensor[{f1[y2[]], f2[y2[]], 0, 0}, {yCoords}, 0][a], 
    {4, 3, 4} -> CTensor[{f1[y2[]], f2[y2[]], 0, 0}, {yCoords}, 0][a], 
    {4, 3, 5} -> CTensor[{f1[y2[]], f2[y2[]], 0, 0}, {yCoords}, 0][a], 
    {4, 3, 6} -> CTensor[{f1[y2[]], f2[y2[]], 0, 0}, {yCoords}, 0][a], 
    {4, 3, 8} -> CTensor[{0, 0, f1[y3[]], f2[y3[]]}, {yCoords}, 0][a], 
    {4, 3, 9} -> CTensor[{0, 0, f1[y4[]], f2[y4[]]}, {yCoords}, 0][a], 
    {4, 3, 10} -> CTensor[{f1[y2[]], f2[y2[]], 0, 0}, {yCoords}, 0][a], 
    {4, 3, 11} -> CTensor[{0, 0, f1[y3[]], f2[y3[]]}, {yCoords}, 0][a], 
    {4, 4, 1} -> CTensor[{f1[] + Cos[y1[]]*Cot[y3[]]*f3[] - 
         Cot[y3[]]*f4[]*Sin[y1[]], f2[], Cos[y1[]]*f4[] + f3[]*Sin[y1[]], 
        Csc[y3[]]*(Cos[y1[]]*f3[] - f4[]*Sin[y1[]])}, {yCoords}, 0][a], 
    {4, 4, 2} -> CTensor[{f1[] + Cos[y1[]]*Coth[y3[]]*f3[] - 
         Coth[y3[]]*f4[]*Sin[y1[]], f2[], Cos[y1[]]*f4[] + f3[]*Sin[y1[]], 
        Cos[y1[]]*Csch[y3[]]*f3[] - Csch[y3[]]*f4[]*Sin[y1[]]}, {yCoords}, 0][
      a], {4, 4, 9} -> CTensor[{f1[] + y3[]*(f3[] + f4[]*y3[]), -2*f4[], 
        f2[], -f3[] - 2*f4[]*y3[]}, {yCoords}, 0][a], 
    {4, 4, 18} -> CTensor[{f1[] + E^y2[]*f4[]*y3[], f2[], f3[]/E^y2[], 
        E^y2[]*f4[]}, {yCoords}, 0][a], {4, 4, 22} -> 
     CTensor[{f1[] + Cos[y2[]]*f3[]*y3[] - f4[]*Sin[y2[]]*y3[], f2[], 
        Cos[y2[]]*f4[] + f3[]*Sin[y2[]], Cos[y2[]]*f3[] - f4[]*Sin[y2[]]}, 
       {yCoords}, 0][a], {5, 4, 1} -> CTensor[{f1[], f2[], 0, 0}, {yCoords}, 
       0][a], {5, 4, 2} -> CTensor[{f1[], f2[], 0, 0}, {yCoords}, 0][a], 
    {5, 4, 3} -> CTensor[{f1[], f2[], 0, 0}, {yCoords}, 0][a], 
    {5, 4, 6} -> CTensor[{f1[], f2[], 0, 0}, {yCoords}, 0][a], 
    {5, 4, 7} -> CTensor[{0, 0, f1[], f2[]}, {yCoords}, 0][a], 
    {6, 3, 1} -> CTensor[{f1[y1[]], 0, 0, 0}, {yCoords}, 0][a], 
    {6, 3, 2} -> CTensor[{f1[y1[]], 0, 0, 0}, {yCoords}, 0][a], 
    {6, 3, 3} -> CTensor[{f1[y1[]], 0, 0, 0}, {yCoords}, 0][a], 
    {6, 3, 4} -> CTensor[{0, 0, 0, f1[y4[]]}, {yCoords}, 0][a], 
    {6, 3, 5} -> CTensor[{0, 0, f1[y3[]], 0}, {yCoords}, 0][a], 
    {6, 3, 6} -> CTensor[{0, 0, 0, f1[y4[]]}, {yCoords}, 0][a], 
    {6, 4, 1} -> 0, {6, 4, 2} -> 0, {6, 4, 3} -> 0, {6, 4, 4} -> 0, 
    {6, 4, 5} -> 0, {7, 4, 1} -> CTensor[{f1[], 0, 0, 0}, {yCoords}, 0][a], 
    {7, 4, 2} -> CTensor[{f1[], 0, 0, 0}, {yCoords}, 0][a], 
    {7, 4, 3} -> CTensor[{0, 0, 0, f1[]}, {yCoords}, 0][a], 
    {7, 4, 4} -> CTensor[{0, 0, 0, f1[]}, {yCoords}, 0][a]|>
ginvmetricarray = 
   <|{3, 2, 1} -> CTensor[{{-\[Phi]1[y1[], y2[]], \[Phi]2[y1[], y2[]], 0, 0}, 
        {\[Phi]2[y1[], y2[]], \[Phi]3[y1[], y2[]], 0, 0}, 
        {0, 0, \[Phi]4[y1[], y2[]], 0}, {0, 0, 0, \[Phi]4[y1[], y2[]]}}, 
       {-yCoords, -yCoords}, 0][-a, -b], {3, 2, 2} -> 
     CTensor[{{-\[Phi]1[y1[], y2[]], \[Phi]2[y1[], y2[]], 0, 0}, 
        {\[Phi]2[y1[], y2[]], \[Phi]3[y1[], y2[]], 0, 0}, 
        {0, 0, \[Phi]4[y1[], y2[]], 0}, {0, 0, 0, Sinh[y3[]]^2*
          \[Phi]4[y1[], y2[]]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {3, 2, 3} -> CTensor[{{-\[Phi]1[y1[], y2[]], \[Phi]2[y1[], y2[]], 0, 0}, 
        {\[Phi]2[y1[], y2[]], \[Phi]3[y1[], y2[]], 0, 0}, 
        {0, 0, \[Phi]4[y1[], y2[]], 0}, {0, 0, 0, Sin[y3[]]^2*
          \[Phi]4[y1[], y2[]]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {3, 2, 4} -> CTensor[{{-\[Phi]1[y3[], y4[]], 0, 0, 0}, 
        {0, \[Phi]1[y3[], y4[]], 0, 0}, {0, 0, \[Phi]2[y3[], y4[]], 
         \[Phi]3[y3[], y4[]]}, {0, 0, \[Phi]3[y3[], y4[]], 
         \[Phi]4[y3[], y4[]]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {3, 2, 5} -> CTensor[{{-(Cosh[y2[]]^2*\[Phi]1[y3[], y4[]]), 0, 0, 0}, 
        {0, \[Phi]1[y3[], y4[]], 0, 0}, {0, 0, \[Phi]2[y3[], y4[]], 
         \[Phi]3[y3[], y4[]]}, {0, 0, \[Phi]3[y3[], y4[]], 
         \[Phi]4[y3[], y4[]]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {3, 3, 2} -> CTensor[{{-\[Phi]1[y3[]], \[Phi]6[y3[]], \[Phi]7[y3[]], 
         \[Phi]8[y3[]]}, {\[Phi]6[y3[]], \[Phi]5[y3[]], \[Phi]9[y3[]], 
         \[Phi]10[y3[]]}, {\[Phi]7[y3[]], \[Phi]9[y3[]], \[Phi]2[y3[]], 
         \[Phi]3[y3[]]}, {\[Phi]8[y3[]], \[Phi]10[y3[]], \[Phi]3[y3[]], 
         \[Phi]4[y3[]]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {3, 3, 3} -> CTensor[{{-\[Phi]1[y2[]], \[Phi]2[y2[]], \[Phi]5[y2[]], 
         y3[]*\[Phi]1[y2[]] + \[Phi]6[y2[]]}, {\[Phi]2[y2[]], \[Phi]3[y2[]], 
         \[Phi]7[y2[]], -(y3[]*\[Phi]2[y2[]]) + \[Phi]8[y2[]]}, 
        {\[Phi]5[y2[]], \[Phi]7[y2[]], \[Phi]4[y2[]], -(y3[]*\[Phi]5[y2[]]) + 
          \[Phi]9[y2[]]}, {y3[]*\[Phi]1[y2[]] + \[Phi]6[y2[]], 
         -(y3[]*\[Phi]2[y2[]]) + \[Phi]8[y2[]], -(y3[]*\[Phi]5[y2[]]) + 
          \[Phi]9[y2[]], -(y3[]^2*\[Phi]1[y2[]]) + \[Phi]10[y2[]] - 
          2*y3[]*\[Phi]6[y2[]]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {3, 3, 8} -> CTensor[{{-\[Phi]1[y2[]], \[Phi]2[y2[]], 
         Cos[y1[]]*\[Phi]6[y2[]] + Sin[y1[]]*\[Phi]8[y2[]], 
         Cosh[y3[]]*\[Phi]1[y2[]] - Sin[y1[]]*Sinh[y3[]]*\[Phi]6[y2[]] + 
          Cos[y1[]]*Sinh[y3[]]*\[Phi]8[y2[]]}, {\[Phi]2[y2[]], \[Phi]3[y2[]], 
         Cos[y1[]]*\[Phi]5[y2[]] + Sin[y1[]]*\[Phi]9[y2[]], 
         -(Cosh[y3[]]*\[Phi]2[y2[]]) - Sin[y1[]]*Sinh[y3[]]*\[Phi]5[y2[]] + 
          Cos[y1[]]*Sinh[y3[]]*\[Phi]9[y2[]]}, 
        {Cos[y1[]]*\[Phi]6[y2[]] + Sin[y1[]]*\[Phi]8[y2[]], 
         Cos[y1[]]*\[Phi]5[y2[]] + Sin[y1[]]*\[Phi]9[y2[]], 
         Cos[y1[]]^2*\[Phi]10[y2[]] + Sin[y1[]]^2*\[Phi]4[y2[]] + 
          Sin[2*y1[]]*\[Phi]7[y2[]], -(Cos[y1[]]*Sin[y1[]]*Sinh[y3[]]*
            \[Phi]10[y2[]]) + Cos[y1[]]*Sin[y1[]]*Sinh[y3[]]*\[Phi]4[y2[]] - 
          Cos[y1[]]*Cosh[y3[]]*\[Phi]6[y2[]] + Cos[2*y1[]]*Sinh[y3[]]*
           \[Phi]7[y2[]] - Cosh[y3[]]*Sin[y1[]]*\[Phi]8[y2[]]}, 
        {Cosh[y3[]]*\[Phi]1[y2[]] - Sin[y1[]]*Sinh[y3[]]*\[Phi]6[y2[]] + 
          Cos[y1[]]*Sinh[y3[]]*\[Phi]8[y2[]], -(Cosh[y3[]]*\[Phi]2[y2[]]) - 
          Sin[y1[]]*Sinh[y3[]]*\[Phi]5[y2[]] + Cos[y1[]]*Sinh[y3[]]*
           \[Phi]9[y2[]], -(Cos[y1[]]*Sin[y1[]]*Sinh[y3[]]*\[Phi]10[y2[]]) + 
          Cos[y1[]]*Sin[y1[]]*Sinh[y3[]]*\[Phi]4[y2[]] - Cos[y1[]]*Cosh[y3[]]*
           \[Phi]6[y2[]] + Cos[2*y1[]]*Sinh[y3[]]*\[Phi]7[y2[]] - 
          Cosh[y3[]]*Sin[y1[]]*\[Phi]8[y2[]], -(Cosh[y3[]]^2*\[Phi]1[y2[]]) + 
          Sin[y1[]]^2*Sinh[y3[]]^2*\[Phi]10[y2[]] + Cos[y1[]]^2*Sinh[y3[]]^2*
           \[Phi]4[y2[]] + Sin[y1[]]*Sinh[2*y3[]]*\[Phi]6[y2[]] - 
          2*Cos[y1[]]*Sin[y1[]]*Sinh[y3[]]^2*\[Phi]7[y2[]] - 
          Cos[y1[]]*Sinh[2*y3[]]*\[Phi]8[y2[]]}}, {-yCoords, -yCoords}, 0][
      -a, -b], {3, 3, 9} -> CTensor[{{-\[Phi]1[y2[]], \[Phi]2[y2[]], 
         Cos[y1[]]*\[Phi]6[y2[]] + Sin[y1[]]*\[Phi]8[y2[]], 
         Cos[y3[]]*\[Phi]1[y2[]] - Sin[y1[]]*Sin[y3[]]*\[Phi]6[y2[]] + 
          Cos[y1[]]*Sin[y3[]]*\[Phi]8[y2[]]}, {\[Phi]2[y2[]], \[Phi]3[y2[]], 
         Cos[y1[]]*\[Phi]5[y2[]] + Sin[y1[]]*\[Phi]9[y2[]], 
         -(Cos[y3[]]*\[Phi]2[y2[]]) - Sin[y1[]]*Sin[y3[]]*\[Phi]5[y2[]] + 
          Cos[y1[]]*Sin[y3[]]*\[Phi]9[y2[]]}, {Cos[y1[]]*\[Phi]6[y2[]] + 
          Sin[y1[]]*\[Phi]8[y2[]], Cos[y1[]]*\[Phi]5[y2[]] + 
          Sin[y1[]]*\[Phi]9[y2[]], -1/2*\[Phi]1[y2[]] + 
          Cos[y1[]]^2*(\[Phi]1[y2[]]/2 + \[Phi]10[y2[]]) + 
          Sin[y1[]]^2*(\[Phi]1[y2[]]/2 + \[Phi]4[y2[]]) + 
          Sin[2*y1[]]*\[Phi]7[y2[]], -(Cos[y1[]]*Cos[y3[]]*\[Phi]6[y2[]]) + 
          Sin[y3[]]*(Cos[y1[]]*Sin[y1[]]*(-\[Phi]10[y2[]] + \[Phi]4[y2[]]) + 
            Cos[2*y1[]]*\[Phi]7[y2[]]) - Cos[y3[]]*Sin[y1[]]*\[Phi]8[y2[]]}, 
        {Cos[y3[]]*\[Phi]1[y2[]] - Sin[y1[]]*Sin[y3[]]*\[Phi]6[y2[]] + 
          Cos[y1[]]*Sin[y3[]]*\[Phi]8[y2[]], -(Cos[y3[]]*\[Phi]2[y2[]]) - 
          Sin[y1[]]*Sin[y3[]]*\[Phi]5[y2[]] + Cos[y1[]]*Sin[y3[]]*
           \[Phi]9[y2[]], -(Cos[y1[]]*Cos[y3[]]*\[Phi]6[y2[]]) + 
          Sin[y3[]]*(Cos[y1[]]*Sin[y1[]]*(-\[Phi]10[y2[]] + \[Phi]4[y2[]]) + 
            Cos[2*y1[]]*\[Phi]7[y2[]]) - Cos[y3[]]*Sin[y1[]]*\[Phi]8[y2[]], 
         -1/4*((3 + Cos[2*y3[]])*\[Phi]1[y2[]]) + 2*Cos[y3[]]*Sin[y1[]]*
           Sin[y3[]]*\[Phi]6[y2[]] + Sin[y3[]]^2*
           (Sin[y1[]]^2*(\[Phi]1[y2[]]/2 + \[Phi]10[y2[]]) + 
            Cos[y1[]]^2*(\[Phi]1[y2[]]/2 + \[Phi]4[y2[]]) - 
            Sin[2*y1[]]*\[Phi]7[y2[]]) - Cos[y1[]]*Sin[2*y3[]]*
           \[Phi]8[y2[]]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {4, 3, 1} -> CTensor[{{-\[Phi]1[y2[]], \[Phi]2[y2[]], 0, 0}, 
        {\[Phi]2[y2[]], \[Phi]3[y2[]], 0, 0}, {0, 0, \[Phi]4[y2[]], 0}, 
        {0, 0, 0, Sinh[y3[]]^2*\[Phi]4[y2[]]}}, {-yCoords, -yCoords}, 0][-a, 
      -b], {4, 3, 2} -> CTensor[{{-\[Phi]1[y2[]], \[Phi]2[y2[]], 0, 
         Cosh[y3[]]*\[Phi]1[y2[]]}, {\[Phi]2[y2[]], \[Phi]3[y2[]], 0, 
         -(Cosh[y3[]]*\[Phi]2[y2[]])}, {0, 0, \[Phi]4[y2[]], 0}, 
        {Cosh[y3[]]*\[Phi]1[y2[]], -(Cosh[y3[]]*\[Phi]2[y2[]]), 0, 
         -(Cosh[y3[]]^2*\[Phi]1[y2[]]) + Sinh[y3[]]^2*\[Phi]4[y2[]]}}, 
       {-yCoords, -yCoords}, 0][-a, -b], {4, 3, 3} -> 
     CTensor[{{-\[Phi]1[y2[]], \[Phi]2[y2[]], 0, 0}, {\[Phi]2[y2[]], 
         \[Phi]3[y2[]], 0, 0}, {0, 0, \[Phi]4[y2[]], 0}, 
        {0, 0, 0, Sin[y3[]]^2*\[Phi]4[y2[]]}}, {-yCoords, -yCoords}, 0][-a, 
      -b], {4, 3, 4} -> CTensor[{{-\[Phi]1[y2[]], \[Phi]2[y2[]], 0, 
         Cos[y3[]]*\[Phi]1[y2[]]}, {\[Phi]2[y2[]], \[Phi]3[y2[]], 0, 
         -(Cos[y3[]]*\[Phi]2[y2[]])}, {0, 0, \[Phi]4[y2[]], 0}, 
        {Cos[y3[]]*\[Phi]1[y2[]], -(Cos[y3[]]*\[Phi]2[y2[]]), 0, 
         -(Cos[y3[]]^2*\[Phi]1[y2[]]) + Sin[y3[]]^2*\[Phi]4[y2[]]}}, 
       {-yCoords, -yCoords}, 0][-a, -b], {4, 3, 5} -> 
     CTensor[{{-\[Phi]1[y2[]], \[Phi]2[y2[]], 0, y3[]*\[Phi]1[y2[]]}, 
        {\[Phi]2[y2[]], \[Phi]3[y2[]], 0, -(y3[]*\[Phi]2[y2[]])}, 
        {0, 0, \[Phi]4[y2[]], 0}, {y3[]*\[Phi]1[y2[]], -(y3[]*\[Phi]2[y2[]]), 
         0, -(y3[]^2*\[Phi]1[y2[]]) + \[Phi]4[y2[]]}}, {-yCoords, -yCoords}, 
       0][-a, -b], {4, 3, 6} -> 
     CTensor[{{-\[Phi]1[y2[]], \[Phi]2[y2[]], 0, 0}, {\[Phi]2[y2[]], 
         \[Phi]3[y2[]], 0, 0}, {0, 0, \[Phi]4[y2[]], 0}, 
        {0, 0, 0, \[Phi]4[y2[]]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {4, 3, 8} -> CTensor[{{-(Cosh[y2[]]^2*\[Phi]1[y3[]]), 0, 0, 0}, 
        {0, \[Phi]1[y3[]], 0, 0}, {0, 0, \[Phi]2[y3[]], \[Phi]3[y3[]]}, 
        {0, 0, \[Phi]3[y3[]], \[Phi]4[y3[]]}}, {-yCoords, -yCoords}, 0][-a, 
      -b], {4, 3, 9} -> 
     CTensor[{{-(Cosh[y2[]]^2*\[Phi]1[y4[]]) + Sinh[y2[]]^2*\[Phi]2[y4[]], 0, 
         Sinh[y2[]]*\[Phi]2[y4[]], Sinh[y2[]]*\[Phi]3[y4[]]}, 
        {0, \[Phi]1[y4[]], 0, 0}, {Sinh[y2[]]*\[Phi]2[y4[]], 0, 
         \[Phi]2[y4[]], \[Phi]3[y4[]]}, {Sinh[y2[]]*\[Phi]3[y4[]], 0, 
         \[Phi]3[y4[]], \[Phi]4[y4[]]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {4, 3, 10} -> CTensor[{{-\[Phi]1[y2[]], \[Phi]2[y2[]], 0, 
         y3[]*\[Phi]1[y2[]]}, {\[Phi]2[y2[]], \[Phi]3[y2[]], 0, 
         -(y3[]*\[Phi]2[y2[]])}, {0, 0, 0, \[Phi]4[y2[]]}, 
        {y3[]*\[Phi]1[y2[]], -(y3[]*\[Phi]2[y2[]]), \[Phi]4[y2[]], 
         -(y3[]^2*\[Phi]1[y2[]])}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {4, 3, 11} -> CTensor[{{-\[Phi]1[y3[]], 0, 0, 0}, {0, \[Phi]1[y3[]], 0, 
         0}, {0, 0, \[Phi]2[y3[]], \[Phi]3[y3[]]}, {0, 0, \[Phi]3[y3[]], 
         \[Phi]4[y3[]]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {4, 4, 1} -> CTensor[{{-\[Phi]1[], \[Phi]2[], Cos[y1[]]*\[Phi]6[] + 
          Sin[y1[]]*\[Phi]8[], Cos[y3[]]*\[Phi]1[] - Sin[y1[]]*Sin[y3[]]*
           \[Phi]6[] + Cos[y1[]]*Sin[y3[]]*\[Phi]8[]}, {\[Phi]2[], \[Phi]3[], 
         Cos[y1[]]*\[Phi]5[] + Sin[y1[]]*\[Phi]9[], -(Cos[y3[]]*\[Phi]2[]) - 
          Sin[y1[]]*Sin[y3[]]*\[Phi]5[] + Cos[y1[]]*Sin[y3[]]*\[Phi]9[]}, 
        {Cos[y1[]]*\[Phi]6[] + Sin[y1[]]*\[Phi]8[], Cos[y1[]]*\[Phi]5[] + 
          Sin[y1[]]*\[Phi]9[], -1/2*\[Phi]1[] + Cos[y1[]]^2*
           (\[Phi]1[]/2 + \[Phi]10[]) + Sin[y1[]]^2*(\[Phi]1[]/2 + 
            \[Phi]4[]) + Sin[2*y1[]]*\[Phi]7[], 
         Sin[y3[]]*(Cos[y1[]]*Sin[y1[]]*(-\[Phi]10[] + \[Phi]4[]) + 
            Cos[2*y1[]]*\[Phi]7[]) + Cos[y3[]]*(-(Cos[y1[]]*\[Phi]6[]) - 
            Sin[y1[]]*\[Phi]8[])}, {Cos[y3[]]*\[Phi]1[] - 
          Sin[y1[]]*Sin[y3[]]*\[Phi]6[] + Cos[y1[]]*Sin[y3[]]*\[Phi]8[], 
         -(Cos[y3[]]*\[Phi]2[]) - Sin[y1[]]*Sin[y3[]]*\[Phi]5[] + 
          Cos[y1[]]*Sin[y3[]]*\[Phi]9[], 
         Sin[y3[]]*(Cos[y1[]]*Sin[y1[]]*(-\[Phi]10[] + \[Phi]4[]) + 
            Cos[2*y1[]]*\[Phi]7[]) + Cos[y3[]]*(-(Cos[y1[]]*\[Phi]6[]) - 
            Sin[y1[]]*\[Phi]8[]), -1/4*((3 + Cos[2*y3[]])*\[Phi]1[]) + 
          Cos[y1[]]^2*Sin[y3[]]^2*(\[Phi]1[]/2 + \[Phi]4[]) + 
          2*Cos[y3[]]*Sin[y1[]]*Sin[y3[]]*\[Phi]6[] + Sin[y3[]]^2*
           (Sin[y1[]]^2*(\[Phi]1[]/2 + \[Phi]10[]) - Sin[2*y1[]]*\[Phi]7[]) - 
          Cos[y1[]]*Sin[2*y3[]]*\[Phi]8[]}}, {-yCoords, -yCoords}, 0][-a, 
      -b], {4, 4, 2} -> CTensor[{{-\[Phi]1[], \[Phi]2[], 
         Cos[y1[]]*\[Phi]6[] + Sin[y1[]]*\[Phi]8[], Cosh[y3[]]*\[Phi]1[] - 
          Sin[y1[]]*Sinh[y3[]]*\[Phi]6[] + Cos[y1[]]*Sinh[y3[]]*\[Phi]8[]}, 
        {\[Phi]2[], \[Phi]3[], Cos[y1[]]*\[Phi]5[] + Sin[y1[]]*\[Phi]9[], 
         -(Cosh[y3[]]*\[Phi]2[]) - Sin[y1[]]*Sinh[y3[]]*\[Phi]5[] + 
          Cos[y1[]]*Sinh[y3[]]*\[Phi]9[]}, {Cos[y1[]]*\[Phi]6[] + 
          Sin[y1[]]*\[Phi]8[], Cos[y1[]]*\[Phi]5[] + Sin[y1[]]*\[Phi]9[], 
         Cos[y1[]]^2*\[Phi]10[] + Sin[y1[]]^2*\[Phi]4[] + 
          Sin[2*y1[]]*\[Phi]7[], -(Cos[y1[]]*Sin[y1[]]*Sinh[y3[]]*
            \[Phi]10[]) + Cos[y1[]]*Sin[y1[]]*Sinh[y3[]]*\[Phi]4[] - 
          Cos[y1[]]*Cosh[y3[]]*\[Phi]6[] + Cos[2*y1[]]*Sinh[y3[]]*\[Phi]7[] - 
          Cosh[y3[]]*Sin[y1[]]*\[Phi]8[]}, {Cosh[y3[]]*\[Phi]1[] - 
          Sin[y1[]]*Sinh[y3[]]*\[Phi]6[] + Cos[y1[]]*Sinh[y3[]]*\[Phi]8[], 
         -(Cosh[y3[]]*\[Phi]2[]) - Sin[y1[]]*Sinh[y3[]]*\[Phi]5[] + 
          Cos[y1[]]*Sinh[y3[]]*\[Phi]9[], -(Cos[y1[]]*Sin[y1[]]*Sinh[y3[]]*
            \[Phi]10[]) + Cos[y1[]]*Sin[y1[]]*Sinh[y3[]]*\[Phi]4[] - 
          Cos[y1[]]*Cosh[y3[]]*\[Phi]6[] + Cos[2*y1[]]*Sinh[y3[]]*\[Phi]7[] - 
          Cosh[y3[]]*Sin[y1[]]*\[Phi]8[], -(Cosh[y3[]]^2*\[Phi]1[]) + 
          Sin[y1[]]^2*Sinh[y3[]]^2*\[Phi]10[] + Cos[y1[]]^2*Sinh[y3[]]^2*
           \[Phi]4[] + Sin[y1[]]*Sinh[2*y3[]]*\[Phi]6[] - 
          2*Cos[y1[]]*Sin[y1[]]*Sinh[y3[]]^2*\[Phi]7[] - 
          Cos[y1[]]*Sinh[2*y3[]]*\[Phi]8[]}}, {-yCoords, -yCoords}, 0][-b, 
      -a], {4, 4, 9} -> 
     CTensor[{{-\[Phi]1[], (y3[]^2*\[Phi]1[])/2 + \[Phi]6[] - y3[]*\[Phi]8[], 
         \[Phi]7[], -(y3[]*\[Phi]1[]) + \[Phi]8[]}, 
        {(y3[]^2*\[Phi]1[])/2 + \[Phi]6[] - y3[]*\[Phi]8[], 
         -1/4*(y3[]^4*\[Phi]1[]) - 2*y3[]*\[Phi]10[] + y3[]^2*\[Phi]4[] + 
          \[Phi]5[] - y3[]^2*\[Phi]6[] + y3[]^3*\[Phi]8[], 
         -(y3[]*\[Phi]3[]) - (y3[]^2*\[Phi]7[])/2 + \[Phi]9[], 
         (y3[]^3*\[Phi]1[])/2 + \[Phi]10[] - y3[]*\[Phi]4[] + 
          y3[]*\[Phi]6[] - (3*y3[]^2*\[Phi]8[])/2}, 
        {\[Phi]7[], -(y3[]*\[Phi]3[]) - (y3[]^2*\[Phi]7[])/2 + \[Phi]9[], 
         \[Phi]2[], \[Phi]3[] + y3[]*\[Phi]7[]}, 
        {-(y3[]*\[Phi]1[]) + \[Phi]8[], (y3[]^3*\[Phi]1[])/2 + \[Phi]10[] - 
          y3[]*\[Phi]4[] + y3[]*\[Phi]6[] - (3*y3[]^2*\[Phi]8[])/2, 
         \[Phi]3[] + y3[]*\[Phi]7[], -(y3[]^2*\[Phi]1[]) + \[Phi]4[] + 
          2*y3[]*\[Phi]8[]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {4, 4, 18} -> CTensor[{{-\[Phi]1[], \[Phi]2[], E^y2[]*\[Phi]5[], 
         y3[]*\[Phi]1[] + \[Phi]6[]/E^y2[]}, {\[Phi]2[], \[Phi]3[], 
         E^y2[]*\[Phi]7[], -(y3[]*\[Phi]2[]) + \[Phi]8[]/E^y2[]}, 
        {E^y2[]*\[Phi]5[], E^y2[]*\[Phi]7[], E^(2*y2[])*\[Phi]4[], 
         -(E^y2[]*y3[]*\[Phi]5[]) + \[Phi]9[]}, 
        {y3[]*\[Phi]1[] + \[Phi]6[]/E^y2[], -(y3[]*\[Phi]2[]) + 
          \[Phi]8[]/E^y2[], -(E^y2[]*y3[]*\[Phi]5[]) + \[Phi]9[], 
         -(y3[]^2*\[Phi]1[]) + \[Phi]10[]/E^(2*y2[]) - (2*y3[]*\[Phi]6[])/
           E^y2[]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {4, 4, 22} -> CTensor[{{-\[Phi]1[], \[Phi]2[], Cos[y2[]]*\[Phi]5[] + 
          Sin[y2[]]*\[Phi]6[], y3[]*\[Phi]1[] - Sin[y2[]]*\[Phi]5[] + 
          Cos[y2[]]*\[Phi]6[]}, {\[Phi]2[], \[Phi]3[], Cos[y2[]]*\[Phi]7[] + 
          Sin[y2[]]*\[Phi]8[], -(y3[]*\[Phi]2[]) - Sin[y2[]]*\[Phi]7[] + 
          Cos[y2[]]*\[Phi]8[]}, {Cos[y2[]]*\[Phi]5[] + Sin[y2[]]*\[Phi]6[], 
         Cos[y2[]]*\[Phi]7[] + Sin[y2[]]*\[Phi]8[], Sin[y2[]]^2*\[Phi]10[] + 
          Cos[y2[]]^2*\[Phi]4[] + Sin[2*y2[]]*\[Phi]9[], 
         Cos[y2[]]*(Sin[y2[]]*(\[Phi]10[] - \[Phi]4[]) - y3[]*\[Phi]5[]) - 
          Sin[y2[]]*y3[]*\[Phi]6[] + Cos[2*y2[]]*\[Phi]9[]}, 
        {y3[]*\[Phi]1[] - Sin[y2[]]*\[Phi]5[] + Cos[y2[]]*\[Phi]6[], 
         -(y3[]*\[Phi]2[]) - Sin[y2[]]*\[Phi]7[] + Cos[y2[]]*\[Phi]8[], 
         Cos[y2[]]*(Sin[y2[]]*(\[Phi]10[] - \[Phi]4[]) - y3[]*\[Phi]5[]) - 
          Sin[y2[]]*y3[]*\[Phi]6[] + Cos[2*y2[]]*\[Phi]9[], 
         -(y3[]^2*\[Phi]1[]) + Cos[y2[]]^2*\[Phi]10[] + 
          Sin[y2[]]^2*\[Phi]4[] + 2*Sin[y2[]]*y3[]*\[Phi]5[] - 
          2*Cos[y2[]]*y3[]*\[Phi]6[] - Sin[2*y2[]]*\[Phi]9[]}}, 
       {-yCoords, -yCoords}, 0][-a, -b], {5, 4, 1} -> 
     CTensor[{{-\[Phi]1[], \[Phi]2[], 0, Cosh[y3[]]*\[Phi]1[]}, 
        {\[Phi]2[], \[Phi]3[], 0, -(Cosh[y3[]]*\[Phi]2[])}, 
        {0, 0, \[Phi]4[], 0}, {Cosh[y3[]]*\[Phi]1[], -(Cosh[y3[]]*\[Phi]2[]), 
         0, -\[Phi]1[] + Sinh[y3[]]^2*(-\[Phi]1[] + \[Phi]4[])}}, 
       {-yCoords, -yCoords}, 0][-a, -b], {5, 4, 2} -> 
     CTensor[{{-\[Phi]1[], \[Phi]2[], 0, 
         -(Cos[y3[]]*(-\[Phi]1[] - \[Phi]4[])) - Cos[y3[]]*\[Phi]4[]}, 
        {\[Phi]2[], \[Phi]3[], 0, -(Cos[y3[]]*\[Phi]2[])}, 
        {0, 0, \[Phi]4[], 0}, {-(Cos[y3[]]*(-\[Phi]1[] - \[Phi]4[])) - 
          Cos[y3[]]*\[Phi]4[], -(Cos[y3[]]*\[Phi]2[]), 0, 
         Cos[y3[]]^2*(-\[Phi]1[] - \[Phi]4[]) + \[Phi]4[]}}, 
       {-yCoords, -yCoords}, 0][-a, -b], {5, 4, 3} -> 
     CTensor[{{-\[Phi]1[], \[Phi]2[], 0, y3[]*\[Phi]1[]}, 
        {\[Phi]2[], \[Phi]3[], 0, -(y3[]*\[Phi]2[])}, {0, 0, \[Phi]4[], 0}, 
        {y3[]*\[Phi]1[], -(y3[]*\[Phi]2[]), 0, -(y3[]^2*\[Phi]1[]) + 
          \[Phi]4[]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {5, 4, 6} -> CTensor[{{-\[Phi]1[], \[Phi]2[], 0, y3[]*\[Phi]1[]}, 
        {\[Phi]2[], \[Phi]3[], 0, -(y3[]*\[Phi]2[])}, {0, 0, 0, \[Phi]4[]}, 
        {y3[]*\[Phi]1[], -(y3[]*\[Phi]2[]), \[Phi]4[], -(y3[]^2*\[Phi]1[])}}, 
       {-yCoords, -yCoords}, 0][-a, -b], {5, 4, 7} -> 
     CTensor[{{-\[Phi]2[] + Cosh[y2[]]^2*(-\[Phi]1[] + \[Phi]2[]), 0, 
         Sinh[y2[]]*\[Phi]2[], Sinh[y2[]]*\[Phi]3[]}, {0, \[Phi]1[], 0, 0}, 
        {Sinh[y2[]]*\[Phi]2[], 0, \[Phi]2[], \[Phi]3[]}, 
        {Sinh[y2[]]*\[Phi]3[], 0, \[Phi]3[], \[Phi]4[]}}, 
       {-yCoords, -yCoords}, 0][-a, -b], {6, 3, 1} -> 
     CTensor[{{-\[Phi]1[y1[]], 0, 0, 0}, {0, \[Phi]2[y1[]], 0, 0}, 
        {0, 0, Sin[y2[]]^2*\[Phi]2[y1[]], 0}, {0, 0, 0, 
         Sin[y2[]]^2*Sin[y3[]]^2*\[Phi]2[y1[]]}}, {-yCoords, -yCoords}, 0][
      -a, -b], {6, 3, 2} -> CTensor[{{-\[Phi]1[y1[]], 0, 0, 0}, 
        {0, \[Phi]2[y1[]], 0, 0}, {0, 0, \[Phi]2[y1[]], 0}, 
        {0, 0, 0, \[Phi]2[y1[]]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {6, 3, 3} -> CTensor[{{-\[Phi]1[y1[]], 0, 0, 0}, {0, \[Phi]2[y1[]], 0, 
         0}, {0, 0, Sinh[y2[]]^2*\[Phi]2[y1[]], 0}, 
        {0, 0, 0, Sin[y3[]]^2*Sinh[y2[]]^2*\[Phi]2[y1[]]}}, 
       {-yCoords, -yCoords}, 0][-a, -b], {6, 3, 4} -> 
     CTensor[{{-(Cosh[y2[]]^2*\[Phi]1[y4[]]), 0, 0, 0}, 
        {0, \[Phi]1[y4[]], 0, 0}, {0, 0, Sinh[y2[]]^2*\[Phi]1[y4[]], 0}, 
        {0, 0, 0, \[Phi]2[y4[]]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {6, 3, 5} -> CTensor[{{-\[Phi]1[y3[]], 0, 0, 0}, {0, \[Phi]1[y3[]], 0, 
         0}, {0, 0, \[Phi]2[y3[]], 0}, {0, 0, 0, \[Phi]1[y3[]]}}, 
       {-yCoords, -yCoords}, 0][-a, -b], {6, 3, 6} -> 
     CTensor[{{-\[Phi]1[y4[]], 0, 0, 0}, {0, Cosh[y1[]]^2*\[Phi]1[y4[]], 0, 
         0}, {0, 0, Cosh[y1[]]^2*Sin[y2[]]^2*\[Phi]1[y4[]], 0}, 
        {0, 0, 0, \[Phi]2[y4[]]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {6, 4, 1} -> CTensor[{{-(Cosh[y2[]]^2*\[Phi]1[]), 0, 0, 0}, 
        {0, \[Phi]1[], 0, 0}, {0, 0, \[Phi]2[], 0}, 
        {0, 0, 0, Sin[y3[]]^2*\[Phi]2[]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {6, 4, 2} -> CTensor[{{-(Cosh[y2[]]^2*\[Phi]1[]), 0, 0, 0}, 
        {0, \[Phi]1[], 0, 0}, {0, 0, \[Phi]2[], 0}, 
        {0, 0, 0, Sinh[y3[]]^2*\[Phi]2[]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {6, 4, 3} -> CTensor[{{-(Cosh[y2[]]^2*\[Phi]1[]), 0, 0, 0}, 
        {0, \[Phi]1[], 0, 0}, {0, 0, \[Phi]2[], 0}, {0, 0, 0, \[Phi]2[]}}, 
       {-yCoords, -yCoords}, 0][-a, -b], {6, 4, 4} -> 
     CTensor[{{-\[Phi]1[], 0, 0, 0}, {0, \[Phi]1[], 0, 0}, 
        {0, 0, \[Phi]2[], 0}, {0, 0, 0, Sin[y3[]]^2*\[Phi]2[]}}, 
       {-yCoords, -yCoords}, 0][-a, -b], {6, 4, 5} -> 
     CTensor[{{-\[Phi]1[], 0, 0, 0}, {0, \[Phi]1[], 0, 0}, 
        {0, 0, \[Phi]2[], 0}, {0, 0, 0, Sinh[y3[]]^2*\[Phi]2[]}}, 
       {-yCoords, -yCoords}, 0][-a, -b], {7, 4, 1} -> 
     CTensor[{{-\[Phi]1[], 0, 0, 0}, {0, \[Phi]2[], 0, 0}, 
        {0, 0, Sin[y2[]]^2*\[Phi]2[], 0}, {0, 0, 0, Sin[y2[]]^2*Sin[y3[]]^2*
          \[Phi]2[]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {7, 4, 2} -> CTensor[{{-\[Phi]1[], 0, 0, 0}, {0, \[Phi]2[], 0, 0}, 
        {0, 0, Sinh[y2[]]^2*\[Phi]2[], 0}, {0, 0, 0, Sin[y3[]]^2*Sinh[y2[]]^2*
          \[Phi]2[]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {7, 4, 3} -> CTensor[{{-\[Phi]1[], 0, 0, 0}, {0, Cosh[y1[]]^2*\[Phi]1[], 
         0, 0}, {0, 0, Cosh[y1[]]^2*Sin[y2[]]^2*\[Phi]1[], 0}, 
        {0, 0, 0, \[Phi]2[]}}, {-yCoords, -yCoords}, 0][-a, -b], 
    {7, 4, 4} -> CTensor[{{-(Cosh[y2[]]^2*\[Phi]1[]), 0, 0, 0}, 
        {0, \[Phi]1[], 0, 0}, {0, 0, Sinh[y2[]]^2*\[Phi]1[], 0}, 
        {0, 0, 0, \[Phi]2[]}}, {-yCoords, -yCoords}, 0][-a, -b]|>
ginvlchainarray = <|{3, 2, 1} -> Basis[{3, -yCoords}, a] \[Wedge] 
      Basis[{4, -yCoords}, b], {3, 2, 2} -> 
     -(Csch[y3[]]*Basis[{3, -yCoords}, a] \[Wedge] Basis[{4, -yCoords}, b]), 
    {3, 2, 3} -> Csc[y3[]]*Basis[{3, -yCoords}, a] \[Wedge] 
       Basis[{4, -yCoords}, b], {3, 2, 4} -> Basis[{1, -yCoords}, a] \[Wedge] 
      Basis[{2, -yCoords}, b], {3, 2, 5} -> 
     -(Sech[y2[]]*Basis[{1, -yCoords}, a] \[Wedge] Basis[{2, -yCoords}, b]), 
    {3, 3, 2} -> Basis[{1, -yCoords}, a] \[Wedge] Basis[{2, -yCoords}, 
       b] \[Wedge] Basis[{4, -yCoords}, c], 
    {3, 3, 3} -> Basis[{1, -yCoords}, a] \[Wedge] Basis[{3, -yCoords}, 
       b] \[Wedge] Basis[{4, -yCoords}, c], 
    {3, 3, 8} -> -2*Csch[y3[]]*Basis[{1, -yCoords}, a] \[Wedge] 
       Basis[{3, -yCoords}, b] \[Wedge] Basis[{4, -yCoords}, c], 
    {3, 3, 9} -> -(Csc[y3[]]*Basis[{1, -yCoords}, a] \[Wedge] 
        Basis[{3, -yCoords}, b] \[Wedge] Basis[{4, -yCoords}, c]), 
    {4, 3, 1} -> Csch[y3[]]*Basis[{1, -yCoords}, a] \[Wedge] 
       Basis[{3, -yCoords}, b] \[Wedge] Basis[{4, -yCoords}, c], 
    {4, 3, 2} -> 2*Csch[y3[]]*Basis[{1, -yCoords}, a] \[Wedge] 
       Basis[{3, -yCoords}, b] \[Wedge] Basis[{4, -yCoords}, c], 
    {4, 3, 3} -> Csc[y3[]]*Basis[{1, -yCoords}, a] \[Wedge] 
       Basis[{3, -yCoords}, b] \[Wedge] Basis[{4, -yCoords}, c], 
    {4, 3, 4} -> -(Csc[y3[]]*Basis[{1, -yCoords}, a] \[Wedge] 
        Basis[{3, -yCoords}, b] \[Wedge] Basis[{4, -yCoords}, c]), 
    {4, 3, 5} -> Basis[{1, -yCoords}, a] \[Wedge] Basis[{3, -yCoords}, 
       b] \[Wedge] Basis[{4, -yCoords}, c], 
    {4, 3, 6} -> -(Basis[{1, -yCoords}, a] \[Wedge] Basis[{3, -yCoords}, 
        b] \[Wedge] Basis[{4, -yCoords}, c]), 
    {4, 3, 8} -> Sech[y2[]]*Basis[{1, -yCoords}, a] \[Wedge] 
       Basis[{2, -yCoords}, b] \[Wedge] Basis[{4, -yCoords}, c], 
    {4, 3, 9} -> -2*Sech[y2[]]*Basis[{1, -yCoords}, a] \[Wedge] 
       Basis[{2, -yCoords}, b] \[Wedge] Basis[{3, -yCoords}, c], 
    {4, 3, 10} -> Basis[{1, -yCoords}, a] \[Wedge] Basis[{3, -yCoords}, 
       b] \[Wedge] Basis[{4, -yCoords}, c], {4, 3, 11} -> 
     Basis[{1, -yCoords}, a] \[Wedge] Basis[{2, -yCoords}, b] \[Wedge] 
      Basis[{4, -yCoords}, c], {4, 4, 1} -> 
     -(Csc[y3[]]*Basis[{1, -yCoords}, a] \[Wedge] Basis[{2, -yCoords}, 
         b] \[Wedge] Basis[{3, -yCoords}, c] \[Wedge] Basis[{4, -yCoords}, 
         d]), {4, 4, 2} -> -2*Csch[y3[]]*Basis[{1, -yCoords}, a] \[Wedge] 
       Basis[{2, -yCoords}, b] \[Wedge] Basis[{3, -yCoords}, c] \[Wedge] 
       Basis[{4, -yCoords}, d], {4, 4, 9} -> 
     -(Basis[{1, -yCoords}, a] \[Wedge] Basis[{2, -yCoords}, b] \[Wedge] 
       Basis[{3, -yCoords}, c] \[Wedge] Basis[{4, -yCoords}, d]), 
    {4, 4, 18} -> Basis[{1, -yCoords}, a] \[Wedge] Basis[{2, -yCoords}, 
       b] \[Wedge] Basis[{3, -yCoords}, c] \[Wedge] Basis[{4, -yCoords}, d], 
    {4, 4, 22} -> Basis[{1, -yCoords}, a] \[Wedge] Basis[{2, -yCoords}, 
       b] \[Wedge] Basis[{3, -yCoords}, c] \[Wedge] Basis[{4, -yCoords}, d], 
    {5, 4, 1} -> 2*Csch[y3[]]*Basis[{1, -yCoords}, a] \[Wedge] 
       Basis[{2, -yCoords}, b] \[Wedge] Basis[{3, -yCoords}, c] \[Wedge] 
       Basis[{4, -yCoords}, d], {5, 4, 2} -> 
     -(Csc[y3[]]*Basis[{1, -yCoords}, a] \[Wedge] Basis[{2, -yCoords}, 
         b] \[Wedge] Basis[{3, -yCoords}, c] \[Wedge] Basis[{4, -yCoords}, 
         d]), {5, 4, 3} -> Basis[{1, -yCoords}, a] \[Wedge] 
      Basis[{2, -yCoords}, b] \[Wedge] Basis[{3, -yCoords}, c] \[Wedge] 
      Basis[{4, -yCoords}, d], {5, 4, 6} -> Basis[{1, -yCoords}, a] \[Wedge] 
      Basis[{2, -yCoords}, b] \[Wedge] Basis[{3, -yCoords}, c] \[Wedge] 
      Basis[{4, -yCoords}, d], {5, 4, 7} -> -2*Sech[y2[]]*
      Basis[{1, -yCoords}, a] \[Wedge] Basis[{2, -yCoords}, b] \[Wedge] 
       Basis[{3, -yCoords}, c] \[Wedge] Basis[{4, -yCoords}, d], 
    {6, 3, 1} -> Csc[y2[]]^2*Csc[y3[]]*Basis[{2, -yCoords}, a] \[Wedge] 
       Basis[{3, -yCoords}, b] \[Wedge] Basis[{4, -yCoords}, c], 
    {6, 3, 2} -> Basis[{2, -yCoords}, a] \[Wedge] Basis[{3, -yCoords}, 
       b] \[Wedge] Basis[{4, -yCoords}, c], 
    {6, 3, 3} -> Csc[y3[]]*Csch[y2[]]^2*Basis[{2, -yCoords}, a] \[Wedge] 
       Basis[{3, -yCoords}, b] \[Wedge] Basis[{4, -yCoords}, c], 
    {6, 3, 4} -> -1/4*(Csch[y2[]]*Sech[y2[]]*Basis[{1, -yCoords}, a] \[Wedge] 
        Basis[{2, -yCoords}, b] \[Wedge] Basis[{3, -yCoords}, c]), 
    {6, 3, 5} -> Basis[{1, -yCoords}, a] \[Wedge] Basis[{2, -yCoords}, 
       b] \[Wedge] Basis[{4, -yCoords}, c], 
    {6, 3, 6} -> -(Csc[y2[]]*Sech[y1[]]^2*Basis[{1, -yCoords}, a] \[Wedge] 
        Basis[{2, -yCoords}, b] \[Wedge] Basis[{3, -yCoords}, c]), 
    {6, 4, 1} -> Csc[y3[]]*Sech[y2[]]*Basis[{1, -yCoords}, a] \[Wedge] 
       Basis[{2, -yCoords}, b] \[Wedge] Basis[{3, -yCoords}, c] \[Wedge] 
       Basis[{4, -yCoords}, d], {6, 4, 2} -> Csch[y3[]]*Sech[y2[]]*
      Basis[{1, -yCoords}, a] \[Wedge] Basis[{2, -yCoords}, b] \[Wedge] 
       Basis[{3, -yCoords}, c] \[Wedge] Basis[{4, -yCoords}, d], 
    {6, 4, 3} -> -(Sech[y2[]]*Basis[{1, -yCoords}, a] \[Wedge] 
        Basis[{2, -yCoords}, b] \[Wedge] Basis[{3, -yCoords}, c] \[Wedge] 
        Basis[{4, -yCoords}, d]), {6, 4, 4} -> 
     -(Csc[y3[]]*Basis[{1, -yCoords}, a] \[Wedge] Basis[{2, -yCoords}, 
         b] \[Wedge] Basis[{3, -yCoords}, c] \[Wedge] Basis[{4, -yCoords}, 
         d]), {6, 4, 5} -> -(Csch[y3[]]*Basis[{1, -yCoords}, a] \[Wedge] 
        Basis[{2, -yCoords}, b] \[Wedge] Basis[{3, -yCoords}, c] \[Wedge] 
        Basis[{4, -yCoords}, d]), {7, 4, 1} -> Csc[y2[]]^2*Csc[y3[]]*
      Basis[{1, -yCoords}, a] \[Wedge] Basis[{2, -yCoords}, b] \[Wedge] 
       Basis[{3, -yCoords}, c] \[Wedge] Basis[{4, -yCoords}, d], 
    {7, 4, 2} -> -(Csc[y3[]]*Csch[y2[]]^2*Basis[{1, -yCoords}, a] \[Wedge] 
        Basis[{2, -yCoords}, b] \[Wedge] Basis[{3, -yCoords}, c] \[Wedge] 
        Basis[{4, -yCoords}, d]), {7, 4, 3} -> 
     -(Csc[y2[]]*Sech[y1[]]^2*Basis[{1, -yCoords}, a] \[Wedge] 
        Basis[{2, -yCoords}, b] \[Wedge] Basis[{3, -yCoords}, c] \[Wedge] 
        Basis[{4, -yCoords}, d]), {7, 4, 4} -> 
     -1/4*(Csch[y2[]]*Sech[y2[]]*Basis[{1, -yCoords}, a] \[Wedge] 
        Basis[{2, -yCoords}, b] \[Wedge] Basis[{3, -yCoords}, c] \[Wedge] 
        Basis[{4, -yCoords}, d])|>
normalizerarray = <|{3, 2, 1} -> {Basis[{1, -yCoords}, a]*f1[y1[], y2[]] + 
       Basis[{2, -yCoords}, a]*f2[y1[], y2[]], Basis[{3, -yCoords}, a]*y3[] + 
       Basis[{4, -yCoords}, a]*y4[], Basis[{4, -yCoords}, a]*y3[] - 
       Basis[{3, -yCoords}, a]*y4[], Basis[{4, -yCoords}, a], 
      -Basis[{3, -yCoords}, a]}, {3, 2, 2} -> 
     {Basis[{1, -yCoords}, a]*f1[y1[], y2[]] + Basis[{2, -yCoords}, a]*
        f2[y1[], y2[]], -Basis[{4, -yCoords}, a], 
      Basis[{4, -yCoords}, a]*Cos[y4[]]*Coth[y3[]] + Basis[{3, -yCoords}, a]*
        Sin[y4[]], Basis[{3, -yCoords}, a]*Cos[y4[]] - 
       Basis[{4, -yCoords}, a]*Coth[y3[]]*Sin[y4[]]}, 
    {3, 2, 3} -> {Basis[{1, -yCoords}, a]*f1[y1[], y2[]] + 
       Basis[{2, -yCoords}, a]*f2[y1[], y2[]], -Basis[{4, -yCoords}, a], 
      -(Basis[{4, -yCoords}, a]*Cos[y4[]]*Cot[y3[]]) - 
       Basis[{3, -yCoords}, a]*Sin[y4[]], 
      -(Basis[{3, -yCoords}, a]*Cos[y4[]]) + Basis[{4, -yCoords}, a]*
        Cot[y3[]]*Sin[y4[]]}, {3, 2, 4} -> 
     {Basis[{3, -yCoords}, a]*f1[y3[], y4[]] + Basis[{4, -yCoords}, a]*
        f2[y3[], y4[]], Basis[{1, -yCoords}, a]*y1[] + 
       Basis[{2, -yCoords}, a]*y2[], Basis[{2, -yCoords}, a]*y1[] + 
       Basis[{1, -yCoords}, a]*y2[], -Basis[{2, -yCoords}, a], 
      -Basis[{1, -yCoords}, a]}, {3, 2, 5} -> 
     {Basis[{3, -yCoords}, a]*f1[y3[], y4[]] + Basis[{4, -yCoords}, a]*
        f2[y3[], y4[]], -Basis[{1, -yCoords}, a], 
      Basis[{2, -yCoords}, a]*Sin[y1[]] + Basis[{1, -yCoords}, a]*Cos[y1[]]*
        Tanh[y2[]], Basis[{2, -yCoords}, a]*Cos[y1[]] - 
       Basis[{1, -yCoords}, a]*Sin[y1[]]*Tanh[y2[]]}, 
    {3, 3, 2} -> {Basis[{3, -yCoords}, a]*f1[y3[]] + Basis[{4, -yCoords}, a]*
        f2[y3[]] + Basis[{2, -yCoords}, a]*f3[y3[]] + Basis[{1, -yCoords}, a]*
        f4[y3[]], Basis[{1, -yCoords}, a]*y1[], Basis[{2, -yCoords}, a]*y1[], 
      Basis[{4, -yCoords}, a]*y1[], Basis[{1, -yCoords}, a]*y2[], 
      Basis[{2, -yCoords}, a]*y2[], Basis[{4, -yCoords}, a]*y2[], 
      Basis[{1, -yCoords}, a]*y4[], Basis[{2, -yCoords}, a]*y4[], 
      Basis[{4, -yCoords}, a]*y4[]}, {3, 3, 3} -> 
     {Basis[{2, -yCoords}, a]*f1[y2[]] + Basis[{1, -yCoords}, a]*f3[y2[]] + 
       Basis[{3, -yCoords}, a]*f4[y2[]] + f2[y2[]]*(Basis[{4, -yCoords}, a] + 
         Basis[{1, -yCoords}, a]*y3[]), Basis[{1, -yCoords}, a]*y1[] + 
       Basis[{3, -yCoords}, a]*y3[], Basis[{1, -yCoords}, a]*y4[], 
      -(Basis[{3, -yCoords}, a]*y3[]) + Basis[{4, -yCoords}, a]*y4[], 
      Basis[{3, -yCoords}, a]*y4[] + (Basis[{1, -yCoords}, a]*y4[]^2)/2, 
      Basis[{1, -yCoords}, a]*y3[], Basis[{4, -yCoords}, a]*y3[] + 
       (Basis[{1, -yCoords}, a]*y3[]^2)/2}, 
    {3, 3, 8} -> {Basis[{2, -yCoords}, a]*f1[y2[]] + Basis[{1, -yCoords}, a]*
        f4[y2[]] + f2[y2[]]*(Basis[{1, -yCoords}, a]*Cos[y1[]]*Coth[y3[]] + 
         Basis[{4, -yCoords}, a]*Cos[y1[]]*Csch[y3[]] + 
         Basis[{3, -yCoords}, a]*Sin[y1[]]) + 
       f3[y2[]]*(Basis[{3, -yCoords}, a]*Cos[y1[]] - 
         (Basis[{4, -yCoords}, a] + Basis[{1, -yCoords}, a]*Cosh[y3[]])*
          Csch[y3[]]*Sin[y1[]]), -Basis[{4, -yCoords}, a], 
      Basis[{4, -yCoords}, a]*Cos[y4[]]*Coth[y3[]] + Basis[{1, -yCoords}, a]*
        Cos[y4[]]*Csch[y3[]] + Basis[{3, -yCoords}, a]*Sin[y4[]], 
      Basis[{3, -yCoords}, a]*Cos[y4[]] - Basis[{4, -yCoords}, a]*Coth[y3[]]*
        Sin[y4[]] - Basis[{1, -yCoords}, a]*Csch[y3[]]*Sin[y4[]]}, 
    {3, 3, 9} -> {Basis[{2, -yCoords}, a]*f1[y2[]] + Basis[{1, -yCoords}, a]*
        f4[y2[]] + f2[y2[]]*(Basis[{1, -yCoords}, a]*Cos[y1[]]*Cot[y3[]] + 
         Basis[{4, -yCoords}, a]*Cos[y1[]]*Csc[y3[]] + 
         Basis[{3, -yCoords}, a]*Sin[y1[]]) + 
       f3[y2[]]*(Basis[{3, -yCoords}, a]*Cos[y1[]] - 
         (Basis[{4, -yCoords}, a] + Basis[{1, -yCoords}, a]*Cos[y3[]])*
          Csc[y3[]]*Sin[y1[]]), -Basis[{4, -yCoords}, a], 
      -(Basis[{4, -yCoords}, a]*Cos[y4[]]*Cot[y3[]]) - 
       Basis[{1, -yCoords}, a]*Cos[y4[]]*Csc[y3[]] - Basis[{3, -yCoords}, a]*
        Sin[y4[]], -(Basis[{3, -yCoords}, a]*Cos[y4[]]) + 
       Basis[{4, -yCoords}, a]*Cot[y3[]]*Sin[y4[]] + Basis[{1, -yCoords}, a]*
        Csc[y3[]]*Sin[y4[]]}, {4, 3, 1} -> 
     {Basis[{1, -yCoords}, a]*f1[y2[]] + Basis[{2, -yCoords}, a]*f2[y2[]], 
      -Basis[{4, -yCoords}, a], Basis[{4, -yCoords}, a]*Cos[y4[]]*
        Coth[y3[]] + Basis[{3, -yCoords}, a]*Sin[y4[]], 
      Basis[{3, -yCoords}, a]*Cos[y4[]] - Basis[{4, -yCoords}, a]*Coth[y3[]]*
        Sin[y4[]], Basis[{1, -yCoords}, a]*y1[]}, 
    {4, 3, 2} -> {Basis[{1, -yCoords}, a]*f1[y2[]] + Basis[{2, -yCoords}, a]*
        f2[y2[]], -Basis[{4, -yCoords}, a], 
      Basis[{4, -yCoords}, a]*Cos[y4[]]*Coth[y3[]] + Basis[{1, -yCoords}, a]*
        Cos[y4[]]*Csch[y3[]] + Basis[{3, -yCoords}, a]*Sin[y4[]], 
      Basis[{3, -yCoords}, a]*Cos[y4[]] - Basis[{4, -yCoords}, a]*Coth[y3[]]*
        Sin[y4[]] - Basis[{1, -yCoords}, a]*Csch[y3[]]*Sin[y4[]]}, 
    {4, 3, 3} -> {Basis[{1, -yCoords}, a]*f1[y2[]] + Basis[{2, -yCoords}, a]*
        f2[y2[]], -Basis[{4, -yCoords}, a], 
      -(Basis[{4, -yCoords}, a]*Cos[y4[]]*Cot[y3[]]) - 
       Basis[{3, -yCoords}, a]*Sin[y4[]], 
      -(Basis[{3, -yCoords}, a]*Cos[y4[]]) + Basis[{4, -yCoords}, a]*
        Cot[y3[]]*Sin[y4[]], Basis[{1, -yCoords}, a]*y1[]}, 
    {4, 3, 4} -> {Basis[{1, -yCoords}, a]*f1[y2[]] + Basis[{2, -yCoords}, a]*
        f2[y2[]], -Basis[{4, -yCoords}, a], 
      -(Basis[{4, -yCoords}, a]*Cos[y4[]]*Cot[y3[]]) - 
       Basis[{1, -yCoords}, a]*Cos[y4[]]*Csc[y3[]] - Basis[{3, -yCoords}, a]*
        Sin[y4[]], -(Basis[{3, -yCoords}, a]*Cos[y4[]]) + 
       Basis[{4, -yCoords}, a]*Cot[y3[]]*Sin[y4[]] + Basis[{1, -yCoords}, a]*
        Csc[y3[]]*Sin[y4[]]}, {4, 3, 5} -> 
     {Basis[{2, -yCoords}, a]*f1[y2[]] + Basis[{1, -yCoords}, a]*f2[y2[]], 
      Basis[{1, -yCoords}, a]*y1[] + (Basis[{3, -yCoords}, a]*y3[])/2 + 
       (Basis[{4, -yCoords}, a]*y4[])/2, Basis[{3, -yCoords}, a] + 
       Basis[{1, -yCoords}, a]*y4[], -(Basis[{4, -yCoords}, a]*y3[]) - 
       (Basis[{1, -yCoords}, a]*y3[]^2)/2 + Basis[{3, -yCoords}, a]*y4[] + 
       (Basis[{1, -yCoords}, a]*y4[]^2)/2, -Basis[{4, -yCoords}, a]}, 
    {4, 3, 6} -> {Basis[{1, -yCoords}, a]*f1[y2[]] + Basis[{2, -yCoords}, a]*
        f2[y2[]], Basis[{3, -yCoords}, a]*y3[] + Basis[{4, -yCoords}, a]*
        y4[], Basis[{4, -yCoords}, a]*y3[] - Basis[{3, -yCoords}, a]*y4[], 
      Basis[{4, -yCoords}, a], -Basis[{3, -yCoords}, a], 
      Basis[{1, -yCoords}, a]*y1[]}, {4, 3, 8} -> 
     {Basis[{3, -yCoords}, a]*f1[y3[]] + Basis[{4, -yCoords}, a]*f2[y3[]], 
      -Basis[{1, -yCoords}, a], Basis[{2, -yCoords}, a]*Sin[y1[]] + 
       Basis[{1, -yCoords}, a]*Cos[y1[]]*Tanh[y2[]], 
      Basis[{2, -yCoords}, a]*Cos[y1[]] - Basis[{1, -yCoords}, a]*Sin[y1[]]*
        Tanh[y2[]], Basis[{4, -yCoords}, a]*y4[]}, 
    {4, 3, 9} -> {Basis[{3, -yCoords}, a]*f1[y4[]] + Basis[{4, -yCoords}, a]*
        f2[y4[]], -Basis[{1, -yCoords}, a], 
      Basis[{3, -yCoords}, a]*Cos[y1[]]*Sech[y2[]] + Basis[{2, -yCoords}, a]*
        Sin[y1[]] + Basis[{1, -yCoords}, a]*Cos[y1[]]*Tanh[y2[]], 
      Basis[{2, -yCoords}, a]*Cos[y1[]] - Basis[{3, -yCoords}, a]*Sech[y2[]]*
        Sin[y1[]] - Basis[{1, -yCoords}, a]*Sin[y1[]]*Tanh[y2[]]}, 
    {4, 3, 10} -> {Basis[{1, -yCoords}, a]*f1[y2[]] + Basis[{2, -yCoords}, a]*
        f2[y2[]], Basis[{1, -yCoords}, a]*y1[] + Basis[{3, -yCoords}, a]*
        y3[], Basis[{3, -yCoords}, a] + Basis[{1, -yCoords}, a]*y4[], 
      -(Basis[{3, -yCoords}, a]*y3[]) + Basis[{4, -yCoords}, a]*y4[], 
      -Basis[{4, -yCoords}, a]}, {4, 3, 11} -> 
     {Basis[{3, -yCoords}, a]*f1[y3[]] + Basis[{4, -yCoords}, a]*f2[y3[]], 
      Basis[{1, -yCoords}, a]*y1[] + Basis[{2, -yCoords}, a]*y2[], 
      Basis[{2, -yCoords}, a]*y1[] + Basis[{1, -yCoords}, a]*y2[], 
      Basis[{4, -yCoords}, a]*y4[], -Basis[{2, -yCoords}, a], 
      -Basis[{1, -yCoords}, a]}, {4, 4, 1} -> 
     {Basis[{2, -yCoords}, a]*f1[] + Basis[{1, -yCoords}, a]*f2[] + 
       f3[]*(Basis[{1, -yCoords}, a]*Cos[y1[]]*Cot[y3[]] + 
         Basis[{4, -yCoords}, a]*Cos[y1[]]*Csc[y3[]] + 
         Basis[{3, -yCoords}, a]*Sin[y1[]]) + 
       f4[]*(Basis[{3, -yCoords}, a]*Cos[y1[]] - 
         (Basis[{4, -yCoords}, a] + Basis[{1, -yCoords}, a]*Cos[y3[]])*
          Csc[y3[]]*Sin[y1[]]), -Basis[{4, -yCoords}, a], 
      -(Basis[{4, -yCoords}, a]*Cos[y4[]]*Cot[y3[]]) - 
       Basis[{1, -yCoords}, a]*Cos[y4[]]*Csc[y3[]] - Basis[{3, -yCoords}, a]*
        Sin[y4[]], -(Basis[{3, -yCoords}, a]*Cos[y4[]]) + 
       Basis[{4, -yCoords}, a]*Cot[y3[]]*Sin[y4[]] + Basis[{1, -yCoords}, a]*
        Csc[y3[]]*Sin[y4[]], Basis[{2, -yCoords}, a]*y2[]}, 
    {4, 4, 2} -> {Basis[{2, -yCoords}, a]*f1[] + Basis[{1, -yCoords}, a]*
        f2[] + f3[]*(Basis[{1, -yCoords}, a]*Cos[y1[]]*Coth[y3[]] + 
         Basis[{4, -yCoords}, a]*Cos[y1[]]*Csch[y3[]] + 
         Basis[{3, -yCoords}, a]*Sin[y1[]]) + 
       f4[]*(Basis[{3, -yCoords}, a]*Cos[y1[]] - 
         (Basis[{4, -yCoords}, a] + Basis[{1, -yCoords}, a]*Cosh[y3[]])*
          Csch[y3[]]*Sin[y1[]]), -Basis[{4, -yCoords}, a], 
      Basis[{4, -yCoords}, a]*Cos[y4[]]*Coth[y3[]] + Basis[{1, -yCoords}, a]*
        Cos[y4[]]*Csch[y3[]] + Basis[{3, -yCoords}, a]*Sin[y4[]], 
      Basis[{3, -yCoords}, a]*Cos[y4[]] - Basis[{4, -yCoords}, a]*Coth[y3[]]*
        Sin[y4[]] - Basis[{1, -yCoords}, a]*Csch[y3[]]*Sin[y4[]], 
      Basis[{2, -yCoords}, a]*y2[]}, {4, 4, 9} -> 
     {Basis[{1, -yCoords}, a]*f1[] + Basis[{3, -yCoords}, a]*f2[] + 
       f3[]*(Basis[{4, -yCoords}, a] - Basis[{1, -yCoords}, a]*y3[]) + 
       f4[]*(Basis[{2, -yCoords}, a] + Basis[{4, -yCoords}, a]*y3[] - 
         (Basis[{1, -yCoords}, a]*y3[]^2)/2), Basis[{1, -yCoords}, a]*y1[] + 
       (Basis[{3, -yCoords}, a]*y3[])/2 + (Basis[{4, -yCoords}, a]*y4[])/2, 
      Basis[{1, -yCoords}, a]*y2[], Basis[{2, -yCoords}, a]*y2[] - 
       (Basis[{3, -yCoords}, a]*y3[])/2 + (Basis[{4, -yCoords}, a]*y4[])/2, 
      Basis[{4, -yCoords}, a]*y2[] - Basis[{1, -yCoords}, a]*y4[], 
      Basis[{1, -yCoords}, a]*y3[], Basis[{2, -yCoords}, a]*y3[] + 
       (Basis[{4, -yCoords}, a]*y3[]^2)/2 - (Basis[{1, -yCoords}, a]*y3[]^3)/
        6, Basis[{4, -yCoords}, a]*y3[] - (Basis[{1, -yCoords}, a]*y3[]^2)/
        2}, {4, 4, 18} -> {Basis[{1, -yCoords}, a]*f1[] + 
       (Basis[{3, -yCoords}, a]*f2[])/E^y2[] + Basis[{2, -yCoords}, a]*f3[] + 
       E^y2[]*f4[]*(Basis[{4, -yCoords}, a] + Basis[{1, -yCoords}, a]*y3[]), 
      Basis[{1, -yCoords}, a]*y1[] + Basis[{3, -yCoords}, a]*y3[], 
      Basis[{3, -yCoords}, a] + Basis[{1, -yCoords}, a]*y4[], 
      -(Basis[{3, -yCoords}, a]*y3[]) + Basis[{4, -yCoords}, a]*y4[], 
      -Basis[{4, -yCoords}, a], Basis[{1, -yCoords}, a]*y2[]}, 
    {4, 4, 22} -> {Basis[{2, -yCoords}, a]*f1[] + Basis[{1, -yCoords}, a]*
        f2[] + f3[]*(Basis[{4, -yCoords}, a]*Cos[y2[]] + 
         Basis[{3, -yCoords}, a]*Sin[y2[]] + Basis[{1, -yCoords}, a]*
          Cos[y2[]]*y3[]) + f4[]*(Basis[{3, -yCoords}, a]*Cos[y2[]] - 
         Sin[y2[]]*(Basis[{4, -yCoords}, a] + Basis[{1, -yCoords}, a]*y3[])), 
      Basis[{1, -yCoords}, a]*y1[] + (Basis[{3, -yCoords}, a]*y3[])/2 + 
       (Basis[{4, -yCoords}, a]*y4[])/2, Basis[{3, -yCoords}, a] + 
       Basis[{1, -yCoords}, a]*y4[], -(Basis[{4, -yCoords}, a]*y3[]) - 
       (Basis[{1, -yCoords}, a]*y3[]^2)/2 + Basis[{3, -yCoords}, a]*y4[] + 
       (Basis[{1, -yCoords}, a]*y4[]^2)/2, -Basis[{4, -yCoords}, a], 
      Basis[{1, -yCoords}, a]*y2[]}, {5, 4, 1} -> 
     {Basis[{1, -yCoords}, a]*f1[] + Basis[{2, -yCoords}, a]*f2[], 
      -Basis[{4, -yCoords}, a], Basis[{4, -yCoords}, a]*Cos[y4[]]*
        Coth[y3[]] + Basis[{1, -yCoords}, a]*Cos[y4[]]*Csch[y3[]] + 
       Basis[{3, -yCoords}, a]*Sin[y4[]], Basis[{3, -yCoords}, a]*Cos[y4[]] - 
       Basis[{4, -yCoords}, a]*Coth[y3[]]*Sin[y4[]] - Basis[{1, -yCoords}, a]*
        Csch[y3[]]*Sin[y4[]], Basis[{1, -yCoords}, a]*y2[], 
      Basis[{2, -yCoords}, a]*y2[]}, {5, 4, 2} -> 
     {Basis[{1, -yCoords}, a]*f1[] + Basis[{2, -yCoords}, a]*f2[], 
      -Basis[{4, -yCoords}, a], -(Basis[{4, -yCoords}, a]*Cos[y4[]]*
         Cot[y3[]]) - Basis[{1, -yCoords}, a]*Cos[y4[]]*Csc[y3[]] - 
       Basis[{3, -yCoords}, a]*Sin[y4[]], 
      -(Basis[{3, -yCoords}, a]*Cos[y4[]]) + Basis[{4, -yCoords}, a]*
        Cot[y3[]]*Sin[y4[]] + Basis[{1, -yCoords}, a]*Csc[y3[]]*Sin[y4[]], 
      Basis[{1, -yCoords}, a]*y2[], Basis[{2, -yCoords}, a]*y2[]}, 
    {5, 4, 3} -> {Basis[{1, -yCoords}, a]*f1[] + Basis[{2, -yCoords}, a]*
        f2[], Basis[{1, -yCoords}, a]*y1[] + (Basis[{3, -yCoords}, a]*y3[])/
        2 + (Basis[{4, -yCoords}, a]*y4[])/2, Basis[{3, -yCoords}, a] + 
       Basis[{1, -yCoords}, a]*y4[], -(Basis[{4, -yCoords}, a]*y3[]) - 
       (Basis[{1, -yCoords}, a]*y3[]^2)/2 + Basis[{3, -yCoords}, a]*y4[] + 
       (Basis[{1, -yCoords}, a]*y4[]^2)/2, -Basis[{4, -yCoords}, a], 
      Basis[{1, -yCoords}, a]*y2[], Basis[{2, -yCoords}, a]*y2[]}, 
    {5, 4, 6} -> {Basis[{1, -yCoords}, a]*f1[] + Basis[{2, -yCoords}, a]*
        f2[], Basis[{1, -yCoords}, a]*y1[] + Basis[{3, -yCoords}, a]*y3[], 
      Basis[{3, -yCoords}, a] + Basis[{1, -yCoords}, a]*y4[], 
      -(Basis[{3, -yCoords}, a]*y3[]) + Basis[{4, -yCoords}, a]*y4[], 
      -Basis[{4, -yCoords}, a], Basis[{1, -yCoords}, a]*y2[], 
      Basis[{2, -yCoords}, a]*y2[]}, {5, 4, 7} -> 
     {Basis[{3, -yCoords}, a]*f1[] + Basis[{4, -yCoords}, a]*f2[], 
      -Basis[{1, -yCoords}, a], Basis[{3, -yCoords}, a]*Cos[y1[]]*
        Sech[y2[]] + Basis[{2, -yCoords}, a]*Sin[y1[]] + 
       Basis[{1, -yCoords}, a]*Cos[y1[]]*Tanh[y2[]], 
      Basis[{2, -yCoords}, a]*Cos[y1[]] - Basis[{3, -yCoords}, a]*Sech[y2[]]*
        Sin[y1[]] - Basis[{1, -yCoords}, a]*Sin[y1[]]*Tanh[y2[]], 
      Basis[{3, -yCoords}, a]*y4[], Basis[{4, -yCoords}, a]*y4[]}, 
    {6, 3, 1} -> {Basis[{1, -yCoords}, a]*f1[y1[]], -Basis[{4, -yCoords}, a], 
      -(Basis[{4, -yCoords}, a]*Cos[y4[]]*Cot[y3[]]) - 
       Basis[{3, -yCoords}, a]*Sin[y4[]], 
      -(Basis[{2, -yCoords}, a]*Cos[y3[]]) + Basis[{3, -yCoords}, a]*
        Cot[y2[]]*Sin[y3[]], Basis[{3, -yCoords}, a]*Cos[y3[]]*Cos[y4[]]*
        Cot[y2[]] + Basis[{2, -yCoords}, a]*Cos[y4[]]*Sin[y3[]] - 
       Basis[{4, -yCoords}, a]*Cot[y2[]]*Csc[y3[]]*Sin[y4[]], 
      -(Basis[{3, -yCoords}, a]*Cos[y4[]]) + Basis[{4, -yCoords}, a]*
        Cot[y3[]]*Sin[y4[]], -(Basis[{4, -yCoords}, a]*Cos[y4[]]*Cot[y2[]]*
         Csc[y3[]]) - Basis[{3, -yCoords}, a]*Cos[y3[]]*Cot[y2[]]*Sin[y4[]] - 
       Basis[{2, -yCoords}, a]*Sin[y3[]]*Sin[y4[]]}, 
    {6, 3, 2} -> {Basis[{1, -yCoords}, a]*f1[y1[]], 
      Basis[{2, -yCoords}, a]*y2[] + Basis[{3, -yCoords}, a]*y3[] + 
       Basis[{4, -yCoords}, a]*y4[], Basis[{4, -yCoords}, a]*y3[] - 
       Basis[{3, -yCoords}, a]*y4[], Basis[{3, -yCoords}, a]*y2[] - 
       Basis[{2, -yCoords}, a]*y3[], Basis[{4, -yCoords}, a]*y2[] - 
       Basis[{2, -yCoords}, a]*y4[], Basis[{4, -yCoords}, a], 
      -Basis[{3, -yCoords}, a], Basis[{2, -yCoords}, a]}, 
    {6, 3, 3} -> {Basis[{1, -yCoords}, a]*f1[y1[]], -Basis[{4, -yCoords}, a], 
      -(Basis[{4, -yCoords}, a]*Cos[y4[]]*Cot[y3[]]) - 
       Basis[{3, -yCoords}, a]*Sin[y4[]], 
      -(Basis[{2, -yCoords}, a]*Cos[y3[]]) + Basis[{3, -yCoords}, a]*
        Coth[y2[]]*Sin[y3[]], Basis[{3, -yCoords}, a]*Cos[y3[]]*Cos[y4[]]*
        Coth[y2[]] + Basis[{2, -yCoords}, a]*Cos[y4[]]*Sin[y3[]] - 
       Basis[{4, -yCoords}, a]*Coth[y2[]]*Csc[y3[]]*Sin[y4[]], 
      -(Basis[{3, -yCoords}, a]*Cos[y4[]]) + Basis[{4, -yCoords}, a]*
        Cot[y3[]]*Sin[y4[]], -(Basis[{4, -yCoords}, a]*Cos[y4[]]*Coth[y2[]]*
         Csc[y3[]]) - Basis[{3, -yCoords}, a]*Cos[y3[]]*Coth[y2[]]*
        Sin[y4[]] - Basis[{2, -yCoords}, a]*Sin[y3[]]*Sin[y4[]]}, 
    {6, 3, 4} -> {Basis[{4, -yCoords}, a]*f1[y4[]], 
      Basis[{1, -yCoords}, a]/2 - Basis[{3, -yCoords}, a]/2, 
      (Basis[{3, -yCoords}, a]*Cos[y1[] - y3[]]*Coth[y2[]])/2 - 
       (Basis[{2, -yCoords}, a]*Sin[y1[] - y3[]])/2 - 
       (Basis[{1, -yCoords}, a]*Cos[y1[] - y3[]]*Tanh[y2[]])/2, 
      (Basis[{2, -yCoords}, a]*Cos[y1[] - y3[]])/2 + 
       (Basis[{3, -yCoords}, a]*Coth[y2[]]*Sin[y1[] - y3[]])/2 - 
       (Basis[{1, -yCoords}, a]*Sin[y1[] - y3[]]*Tanh[y2[]])/2, 
      -1/2*Basis[{1, -yCoords}, a] - Basis[{3, -yCoords}, a]/2, 
      -1/2*(Basis[{3, -yCoords}, a]*Cos[y1[] + y3[]]*Coth[y2[]]) - 
       (Basis[{2, -yCoords}, a]*Sin[y1[] + y3[]])/2 - 
       (Basis[{1, -yCoords}, a]*Cos[y1[] + y3[]]*Tanh[y2[]])/2, 
      -1/2*(Basis[{2, -yCoords}, a]*Cos[y1[] + y3[]]) + 
       (Basis[{3, -yCoords}, a]*Coth[y2[]]*Sin[y1[] + y3[]])/2 + 
       (Basis[{1, -yCoords}, a]*Sin[y1[] + y3[]]*Tanh[y2[]])/2}, 
    {6, 3, 5} -> {Basis[{3, -yCoords}, a]*f1[y3[]], 
      Basis[{1, -yCoords}, a]*y1[] + Basis[{2, -yCoords}, a]*y2[] + 
       Basis[{4, -yCoords}, a]*y4[], Basis[{2, -yCoords}, a]*y1[] + 
       Basis[{1, -yCoords}, a]*y2[], Basis[{4, -yCoords}, a]*y1[] + 
       Basis[{1, -yCoords}, a]*y4[], Basis[{4, -yCoords}, a]*y2[] - 
       Basis[{2, -yCoords}, a]*y4[], -Basis[{2, -yCoords}, a], 
      -Basis[{1, -yCoords}, a], -Basis[{4, -yCoords}, a]}, 
    {6, 3, 6} -> {Basis[{4, -yCoords}, a]*f1[y4[]], -Basis[{3, -yCoords}, a], 
      -(Basis[{3, -yCoords}, a]*Cos[y3[]]*Cot[y2[]]) - 
       Basis[{2, -yCoords}, a]*Sin[y3[]], 
      -(Basis[{1, -yCoords}, a]*Cos[y2[]]) + Basis[{2, -yCoords}, a]*
        Sin[y2[]]*Tanh[y1[]], Basis[{1, -yCoords}, a]*Cos[y3[]]*Sin[y2[]] + 
       Basis[{2, -yCoords}, a]*Cos[y2[]]*Cos[y3[]]*Tanh[y1[]] - 
       Basis[{3, -yCoords}, a]*Csc[y2[]]*Sin[y3[]]*Tanh[y1[]], 
      -(Basis[{2, -yCoords}, a]*Cos[y3[]]) + Basis[{3, -yCoords}, a]*
        Cot[y2[]]*Sin[y3[]], -(Basis[{1, -yCoords}, a]*Sin[y2[]]*Sin[y3[]]) - 
       Basis[{3, -yCoords}, a]*Cos[y3[]]*Csc[y2[]]*Tanh[y1[]] - 
       Basis[{2, -yCoords}, a]*Cos[y2[]]*Sin[y3[]]*Tanh[y1[]]}, 
    {6, 4, 1} -> {0, -(Basis[{4, -yCoords}, a]*Cos[y4[]]^2) - 
       Basis[{4, -yCoords}, a]*Sin[y4[]]^2, 
      -(Basis[{4, -yCoords}, a]*Cos[y4[]]*Cot[y3[]]) - 
       Basis[{3, -yCoords}, a]*Cos[y3[]]^2*Sin[y4[]] - 
       Basis[{3, -yCoords}, a]*Sin[y3[]]^2*Sin[y4[]], 
      -(Basis[{3, -yCoords}, a]*Cos[y3[]]^2*Cos[y4[]]) - 
       Basis[{3, -yCoords}, a]*Cos[y4[]]*Sin[y3[]]^2 + 
       Basis[{4, -yCoords}, a]*Cot[y3[]]*Sin[y4[]], 
      -(Basis[{1, -yCoords}, a]*Cos[y1[]]^2) - Basis[{1, -yCoords}, a]*
        Sin[y1[]]^2, Basis[{2, -yCoords}, a]*Cosh[y2[]]^2*Sin[y1[]] - 
       Basis[{2, -yCoords}, a]*Sin[y1[]]*Sinh[y2[]]^2 + 
       Basis[{1, -yCoords}, a]*Cos[y1[]]*Tanh[y2[]], 
      Basis[{2, -yCoords}, a]*Cos[y1[]]*Cosh[y2[]]^2 - 
       Basis[{2, -yCoords}, a]*Cos[y1[]]*Sinh[y2[]]^2 - 
       Basis[{1, -yCoords}, a]*Sin[y1[]]*Tanh[y2[]]}, 
    {6, 4, 2} -> {0, -(Basis[{4, -yCoords}, a]*Cos[y4[]]^2) - 
       Basis[{4, -yCoords}, a]*Sin[y4[]]^2, 
      Basis[{4, -yCoords}, a]*Cos[y4[]]*Coth[y3[]] + Basis[{3, -yCoords}, a]*
        Cosh[y3[]]^2*Sin[y4[]] - Basis[{3, -yCoords}, a]*Sin[y4[]]*
        Sinh[y3[]]^2, Basis[{3, -yCoords}, a]*Cos[y4[]]*Cosh[y3[]]^2 - 
       Basis[{4, -yCoords}, a]*Coth[y3[]]*Sin[y4[]] - Basis[{3, -yCoords}, a]*
        Cos[y4[]]*Sinh[y3[]]^2, -(Basis[{1, -yCoords}, a]*Cos[y1[]]^2) - 
       Basis[{1, -yCoords}, a]*Sin[y1[]]^2, 
      Basis[{2, -yCoords}, a]*Cosh[y2[]]^2*Sin[y1[]] - 
       Basis[{2, -yCoords}, a]*Sin[y1[]]*Sinh[y2[]]^2 + 
       Basis[{1, -yCoords}, a]*Cos[y1[]]*Tanh[y2[]], 
      Basis[{2, -yCoords}, a]*Cos[y1[]]*Cosh[y2[]]^2 - 
       Basis[{2, -yCoords}, a]*Cos[y1[]]*Sinh[y2[]]^2 - 
       Basis[{1, -yCoords}, a]*Sin[y1[]]*Tanh[y2[]]}, 
    {6, 4, 3} -> {0, -(Basis[{1, -yCoords}, a]*Cos[y1[]]^2) - 
       Basis[{1, -yCoords}, a]*Sin[y1[]]^2, 
      Basis[{2, -yCoords}, a]*Cosh[y2[]]^2*Sin[y1[]] - 
       Basis[{2, -yCoords}, a]*Sin[y1[]]*Sinh[y2[]]^2 + 
       Basis[{1, -yCoords}, a]*Cos[y1[]]*Tanh[y2[]], 
      Basis[{2, -yCoords}, a]*Cos[y1[]]*Cosh[y2[]]^2 - 
       Basis[{2, -yCoords}, a]*Cos[y1[]]*Sinh[y2[]]^2 - 
       Basis[{1, -yCoords}, a]*Sin[y1[]]*Tanh[y2[]], 
      Basis[{3, -yCoords}, a]*y3[] + Basis[{4, -yCoords}, a]*y4[], 
      Basis[{4, -yCoords}, a]*y3[] - Basis[{3, -yCoords}, a]*y4[], 
      Basis[{4, -yCoords}, a], -Basis[{3, -yCoords}, a]}, 
    {6, 4, 4} -> {0, -(Basis[{4, -yCoords}, a]*Cos[y4[]]^2) - 
       Basis[{4, -yCoords}, a]*Sin[y4[]]^2, 
      -(Basis[{4, -yCoords}, a]*Cos[y4[]]*Cot[y3[]]) - 
       Basis[{3, -yCoords}, a]*Cos[y3[]]^2*Sin[y4[]] - 
       Basis[{3, -yCoords}, a]*Sin[y3[]]^2*Sin[y4[]], 
      -(Basis[{3, -yCoords}, a]*Cos[y3[]]^2*Cos[y4[]]) - 
       Basis[{3, -yCoords}, a]*Cos[y4[]]*Sin[y3[]]^2 + 
       Basis[{4, -yCoords}, a]*Cot[y3[]]*Sin[y4[]], 
      Basis[{1, -yCoords}, a]*y1[] + Basis[{2, -yCoords}, a]*y2[], 
      Basis[{2, -yCoords}, a]*y1[] + Basis[{1, -yCoords}, a]*y2[], 
      -Basis[{2, -yCoords}, a], -Basis[{1, -yCoords}, a]}, 
    {6, 4, 5} -> {0, -(Basis[{4, -yCoords}, a]*Cos[y4[]]^2) - 
       Basis[{4, -yCoords}, a]*Sin[y4[]]^2, 
      Basis[{4, -yCoords}, a]*Cos[y4[]]*Coth[y3[]] + Basis[{3, -yCoords}, a]*
        Cosh[y3[]]^2*Sin[y4[]] - Basis[{3, -yCoords}, a]*Sin[y4[]]*
        Sinh[y3[]]^2, Basis[{3, -yCoords}, a]*Cos[y4[]]*Cosh[y3[]]^2 - 
       Basis[{4, -yCoords}, a]*Coth[y3[]]*Sin[y4[]] - Basis[{3, -yCoords}, a]*
        Cos[y4[]]*Sinh[y3[]]^2, -Basis[{2, -yCoords}, a], 
      -Basis[{1, -yCoords}, a], Basis[{1, -yCoords}, a]*y1[] + 
       Basis[{2, -yCoords}, a]*y2[], Basis[{2, -yCoords}, a]*y1[] + 
       Basis[{1, -yCoords}, a]*y2[]}, {7, 4, 1} -> 
     {Basis[{1, -yCoords}, a]*f1[], -Basis[{4, -yCoords}, a], 
      -(Basis[{4, -yCoords}, a]*Cos[y4[]]*Cot[y3[]]) - 
       Basis[{3, -yCoords}, a]*Sin[y4[]], 
      -(Basis[{2, -yCoords}, a]*Cos[y3[]]) + Basis[{3, -yCoords}, a]*
        Cot[y2[]]*Sin[y3[]], Basis[{3, -yCoords}, a]*Cos[y3[]]*Cos[y4[]]*
        Cot[y2[]] + Basis[{2, -yCoords}, a]*Cos[y4[]]*Sin[y3[]] - 
       Basis[{4, -yCoords}, a]*Cot[y2[]]*Csc[y3[]]*Sin[y4[]], 
      -(Basis[{3, -yCoords}, a]*Cos[y4[]]) + Basis[{4, -yCoords}, a]*
        Cot[y3[]]*Sin[y4[]], -(Basis[{4, -yCoords}, a]*Cos[y4[]]*Cot[y2[]]*
         Csc[y3[]]) - Basis[{3, -yCoords}, a]*Cos[y3[]]*Cot[y2[]]*Sin[y4[]] - 
       Basis[{2, -yCoords}, a]*Sin[y3[]]*Sin[y4[]], Basis[{1, -yCoords}, a]*
       y1[]}, {7, 4, 2} -> {Basis[{1, -yCoords}, a]*f1[], 
      -Basis[{4, -yCoords}, a], -(Basis[{4, -yCoords}, a]*Cos[y4[]]*
         Cot[y3[]]) - Basis[{3, -yCoords}, a]*Sin[y4[]], 
      -(Basis[{2, -yCoords}, a]*Cos[y3[]]) + Basis[{3, -yCoords}, a]*
        Coth[y2[]]*Sin[y3[]], Basis[{3, -yCoords}, a]*Cos[y3[]]*Cos[y4[]]*
        Coth[y2[]] + Basis[{2, -yCoords}, a]*Cos[y4[]]*Sin[y3[]] - 
       Basis[{4, -yCoords}, a]*Coth[y2[]]*Csc[y3[]]*Sin[y4[]], 
      -(Basis[{3, -yCoords}, a]*Cos[y4[]]) + Basis[{4, -yCoords}, a]*
        Cot[y3[]]*Sin[y4[]], -(Basis[{4, -yCoords}, a]*Cos[y4[]]*Coth[y2[]]*
         Csc[y3[]]) - Basis[{3, -yCoords}, a]*Cos[y3[]]*Coth[y2[]]*
        Sin[y4[]] - Basis[{2, -yCoords}, a]*Sin[y3[]]*Sin[y4[]], 
      Basis[{1, -yCoords}, a]*y1[]}, {7, 4, 3} -> 
     {Basis[{4, -yCoords}, a]*f1[], -Basis[{3, -yCoords}, a], 
      -(Basis[{3, -yCoords}, a]*Cos[y3[]]*Cot[y2[]]) - 
       Basis[{2, -yCoords}, a]*Sin[y3[]], 
      -(Basis[{1, -yCoords}, a]*Cos[y2[]]) + Basis[{2, -yCoords}, a]*
        Sin[y2[]]*Tanh[y1[]], Basis[{1, -yCoords}, a]*Cos[y3[]]*Sin[y2[]] + 
       Basis[{2, -yCoords}, a]*Cos[y2[]]*Cos[y3[]]*Tanh[y1[]] - 
       Basis[{3, -yCoords}, a]*Csc[y2[]]*Sin[y3[]]*Tanh[y1[]], 
      -(Basis[{2, -yCoords}, a]*Cos[y3[]]) + Basis[{3, -yCoords}, a]*
        Cot[y2[]]*Sin[y3[]], -(Basis[{1, -yCoords}, a]*Sin[y2[]]*Sin[y3[]]) - 
       Basis[{3, -yCoords}, a]*Cos[y3[]]*Csc[y2[]]*Tanh[y1[]] - 
       Basis[{2, -yCoords}, a]*Cos[y2[]]*Sin[y3[]]*Tanh[y1[]], 
      Basis[{4, -yCoords}, a]*y4[]}, {7, 4, 4} -> 
     {Basis[{4, -yCoords}, a]*f1[], Basis[{1, -yCoords}, a]/2 - 
       Basis[{3, -yCoords}, a]/2, (Basis[{3, -yCoords}, a]*Cos[y1[] - y3[]]*
         Coth[y2[]])/2 - (Basis[{2, -yCoords}, a]*Sin[y1[] - y3[]])/2 - 
       (Basis[{1, -yCoords}, a]*Cos[y1[] - y3[]]*Tanh[y2[]])/2, 
      (Basis[{2, -yCoords}, a]*Cos[y1[] - y3[]])/2 + 
       (Basis[{3, -yCoords}, a]*Coth[y2[]]*Sin[y1[] - y3[]])/2 - 
       (Basis[{1, -yCoords}, a]*Sin[y1[] - y3[]]*Tanh[y2[]])/2, 
      -1/2*Basis[{1, -yCoords}, a] - Basis[{3, -yCoords}, a]/2, 
      -1/2*(Basis[{3, -yCoords}, a]*Cos[y1[] + y3[]]*Coth[y2[]]) - 
       (Basis[{2, -yCoords}, a]*Sin[y1[] + y3[]])/2 - 
       (Basis[{1, -yCoords}, a]*Cos[y1[] + y3[]]*Tanh[y2[]])/2, 
      -1/2*(Basis[{2, -yCoords}, a]*Cos[y1[] + y3[]]) + 
       (Basis[{3, -yCoords}, a]*Coth[y2[]]*Sin[y1[] + y3[]])/2 + 
       (Basis[{1, -yCoords}, a]*Sin[y1[] + y3[]]*Tanh[y2[]])/2, 
      Basis[{4, -yCoords}, a]*y4[]}|>
nonginvresdiffarray = <|{3, 2, 1} -> {Basis[{3, -yCoords}, a]*y3[] + 
       Basis[{4, -yCoords}, a]*y4[]}, {3, 2, 2} -> {}, {3, 2, 3} -> {}, 
    {3, 2, 4} -> {Basis[{1, -yCoords}, a]*y1[] + Basis[{2, -yCoords}, a]*
        y2[]}, {3, 2, 5} -> {}, {3, 3, 2} -> {Basis[{1, -yCoords}, a]*y1[], 
      Basis[{2, -yCoords}, a]*y1[], Basis[{4, -yCoords}, a]*y1[], 
      Basis[{1, -yCoords}, a]*y2[], Basis[{2, -yCoords}, a]*y2[], 
      Basis[{4, -yCoords}, a]*y2[], Basis[{1, -yCoords}, a]*y4[], 
      Basis[{2, -yCoords}, a]*y4[], Basis[{4, -yCoords}, a]*y4[]}, 
    {3, 3, 3} -> {Basis[{1, -yCoords}, a]*y1[] + Basis[{3, -yCoords}, a]*
        y3[], Basis[{1, -yCoords}, a]*y4[], -(Basis[{3, -yCoords}, a]*y3[]) + 
       Basis[{4, -yCoords}, a]*y4[], Basis[{3, -yCoords}, a]*y4[] + 
       (Basis[{1, -yCoords}, a]*y4[]^2)/2, Basis[{1, -yCoords}, a]*y3[], 
      Basis[{4, -yCoords}, a]*y3[] + (Basis[{1, -yCoords}, a]*y3[]^2)/2}, 
    {3, 3, 8} -> {}, {3, 3, 9} -> {}, {4, 3, 1} -> 
     {Basis[{1, -yCoords}, a]*y1[]}, {4, 3, 2} -> {}, 
    {4, 3, 3} -> {Basis[{1, -yCoords}, a]*y1[]}, {4, 3, 4} -> {}, 
    {4, 3, 5} -> {Basis[{1, -yCoords}, a]*y1[] + 
       (Basis[{3, -yCoords}, a]*y3[])/2 + (Basis[{4, -yCoords}, a]*y4[])/2}, 
    {4, 3, 6} -> {Basis[{3, -yCoords}, a]*y3[] + Basis[{4, -yCoords}, a]*
        y4[], Basis[{1, -yCoords}, a]*y1[]}, 
    {4, 3, 8} -> {Basis[{4, -yCoords}, a]*y4[]}, {4, 3, 9} -> {}, 
    {4, 3, 10} -> {Basis[{1, -yCoords}, a]*y1[] + Basis[{3, -yCoords}, a]*
        y3[]}, {4, 3, 11} -> {Basis[{1, -yCoords}, a]*y1[] + 
       Basis[{2, -yCoords}, a]*y2[], Basis[{4, -yCoords}, a]*y4[]}, 
    {4, 4, 1} -> {Basis[{2, -yCoords}, a]*y2[]}, 
    {4, 4, 2} -> {Basis[{2, -yCoords}, a]*y2[]}, 
    {4, 4, 9} -> {Basis[{1, -yCoords}, a]*y1[] + 
       (Basis[{3, -yCoords}, a]*y3[])/2 + (Basis[{4, -yCoords}, a]*y4[])/2, 
      Basis[{1, -yCoords}, a]*y2[], Basis[{2, -yCoords}, a]*y2[] - 
       (Basis[{3, -yCoords}, a]*y3[])/2 + (Basis[{4, -yCoords}, a]*y4[])/2, 
      Basis[{4, -yCoords}, a]*y2[] - Basis[{1, -yCoords}, a]*y4[], 
      Basis[{1, -yCoords}, a]*y3[], Basis[{2, -yCoords}, a]*y3[] + 
       (Basis[{4, -yCoords}, a]*y3[]^2)/2 - (Basis[{1, -yCoords}, a]*y3[]^3)/
        6, Basis[{4, -yCoords}, a]*y3[] - (Basis[{1, -yCoords}, a]*y3[]^2)/
        2}, {4, 4, 18} -> {Basis[{1, -yCoords}, a]*y1[] + 
       Basis[{3, -yCoords}, a]*y3[], -(Basis[{3, -yCoords}, a]*y3[]) + 
       Basis[{4, -yCoords}, a]*y4[], Basis[{1, -yCoords}, a]*y2[]}, 
    {4, 4, 22} -> {Basis[{1, -yCoords}, a]*y1[] + 
       (Basis[{3, -yCoords}, a]*y3[])/2 + (Basis[{4, -yCoords}, a]*y4[])/2, 
      -(Basis[{4, -yCoords}, a]*y3[]) - (Basis[{1, -yCoords}, a]*y3[]^2)/2 + 
       Basis[{3, -yCoords}, a]*y4[] + (Basis[{1, -yCoords}, a]*y4[]^2)/2, 
      Basis[{1, -yCoords}, a]*y2[]}, {5, 4, 1} -> 
     {Basis[{1, -yCoords}, a]*y2[], Basis[{2, -yCoords}, a]*y2[]}, 
    {5, 4, 2} -> {Basis[{1, -yCoords}, a]*y2[], Basis[{2, -yCoords}, a]*
       y2[]}, {5, 4, 3} -> {Basis[{1, -yCoords}, a]*y1[] + 
       (Basis[{3, -yCoords}, a]*y3[])/2 + (Basis[{4, -yCoords}, a]*y4[])/2, 
      Basis[{1, -yCoords}, a]*y2[], Basis[{2, -yCoords}, a]*y2[]}, 
    {5, 4, 6} -> {Basis[{1, -yCoords}, a]*y1[] + Basis[{3, -yCoords}, a]*
        y3[], Basis[{1, -yCoords}, a]*y2[], Basis[{2, -yCoords}, a]*y2[]}, 
    {5, 4, 7} -> {Basis[{3, -yCoords}, a]*y4[], Basis[{4, -yCoords}, a]*
       y4[]}, {6, 3, 1} -> {}, {6, 3, 2} -> 
     {Basis[{2, -yCoords}, a]*y2[] + Basis[{3, -yCoords}, a]*y3[] + 
       Basis[{4, -yCoords}, a]*y4[]}, {6, 3, 3} -> {}, {6, 3, 4} -> {}, 
    {6, 3, 5} -> {Basis[{1, -yCoords}, a]*y1[] + Basis[{2, -yCoords}, a]*
        y2[] + Basis[{4, -yCoords}, a]*y4[]}, {6, 3, 6} -> {}, 
    {6, 4, 1} -> {}, {6, 4, 2} -> {}, {6, 4, 3} -> 
     {Basis[{3, -yCoords}, a]*y3[] + Basis[{4, -yCoords}, a]*y4[]}, 
    {6, 4, 4} -> {Basis[{1, -yCoords}, a]*y1[] + Basis[{2, -yCoords}, a]*
        y2[]}, {6, 4, 5} -> {Basis[{1, -yCoords}, a]*y1[] + 
       Basis[{2, -yCoords}, a]*y2[]}, {7, 4, 1} -> 
     {Basis[{1, -yCoords}, a]*y1[]}, {7, 4, 2} -> 
     {Basis[{1, -yCoords}, a]*y1[]}, {7, 4, 3} -> 
     {Basis[{4, -yCoords}, a]*y4[]}, {7, 4, 4} -> 
     {Basis[{4, -yCoords}, a]*y4[]}|>

